Locating ballot drop boxes

For decades, voting-by-mail and the use of ballot drop boxes has substantially grown, and in response, many election officials have added new drop boxes to their voting infrastructure. However, existing guidance for locating drop boxes is limited. In this paper, we introduce an integer programming model, the drop box location problem (DBLP), to locate drop boxes. The DBLP considers criteria of cost, voter access, and risk. The cost of the drop box system is determined by the fixed cost of adding drop boxes and the operational cost of a collection tour by a bipartisan team who regularly collects ballots from selected locations. The DBLP utilizes covering sets to ensure each voter is in close proximity to a drop box and incorporates a novel measure of access to measure the ability to use multiple voting pathways to vote. The DBLP is shown to be NP-Hard, and we introduce a heuristic to generate a large number of feasible solutions for policy makers to select from a posteriori. Using a real-world case study of Milwaukee, WI, we study the benefit of the DBLP. The results demonstrate that the proposed optimization model identifies drop box locations that perform well across multiple criteria. The results also demonstrate that the trade-off between cost, access, and risk is non-trivial, which supports the use of the proposed optimization-based approach to select drop box locations.

==> heuristic_writeup.tex <==
\section{Heuristic Method and Results}

The DBLP is shown to be NP-Hard. 
% In response, we introduce a polynomial-time local search heuristic algorithm to identify feasible solutions to the DBLP that approximate the Pareto frontier corresponding to the objectives to maximize access and minimize cost.
In response, we introduce a polynomial-time, local search heuristic algorithm that approximates the Pareto frontier corresponding to access and cost while ensuring that risks are mitigated using constraints.
This heuristic can be executed for different input parameters to understand the impact of varying risk tolerance.
The heuristic operates by first finding a near-minimal cost solution to the DBLP by relaxing the DBLP to produce an instance of the CTP. 
% Then, any existing algorithm for the CTP is used as a subroutine to identify an initial feasible solution to the DBLP. 
Starting from this initial DBLP solution, a series of swaps are identified to determine drop box locations that progressively yields solutions that admit higher access. 
The collection of solutions illuminate the trade-offs of the drop box system to election administrators.


% \section{Heuristic Solution Method}\label{sec:heuristic}
When the RHS of constraint set \eqref{model:basecoverage} is one, we only need to solve the CTP once.
When the RHS is zero, the subproblem is just a TSP that can be solved.

'Value' thing is simiar to apprach used by \citet{gendreau_covering_1997} except their value is for coverage set.




\textcolor{red}{Shorten this}
The TSP, which is NP-Hard, can be reduced to the DBLP when $r = 0$, $N_w = \emptyset$ for $w \in W$, and $T = V$.
Thus, the DBLP is also NP-Hard.
% The DBLP can also be reduced to a set covering-ike problem when $c_{ij} = 0$ for each $i\in N$ and $j \in N$, which is also NP-Hard. %
This motivates the need to find a heuristic solution algorithm that identifies feasible solutions in polynomial time. 
A challenge of the  DBLP is its multi-objective form. The collection of desired solutions lie on a Pareto frontier.
% In response, t
The heuristic method we introduce seeks to identify a collection of non-dominated solutions that approximates the Pareto frontier corresponding to access and cost.
The heuristic method can be re-executed for different risk-based inputs to provide insight into the trade-off between access, cost, and risk.
% that would result from a unique preference for each objective. 
Election administrators can select from these solutions a posterirori.
% We address the case where a collection of solutions must be obtained for election administrators or policy makers to select from a posteriori.
This is an advantage for practice as it allows election adminitrators better assess the trade-off between potential drop box locations.



% The heuristic method we introduce generates multiple feasible solutions to the DBLP that lie near the Pareto frontier.
% Within this section, we consider the reformulation of the first objective $z_1$ as introduced in Section \ref{sec:obj1reform}.
% Additionally, the heuristic algorithm makes use of the alternative form of the access function as described by equation \eqref{reformcoverage} in Section \ref{sec:obj2reform}.
% With this reformulation, the second objective is to minimize equation $z_2$.

Our heuristic solution method has two main steps. 
In the first step, we find a feasible solution to the DBLP of roughly minimal cost, $z_1$, while ignoring the access function constraint set \eqref{model:obj2}.
This step is completed only once during the solution procedure.
The second step repeats in an iterative fashion.
In an iteration of the second step, we identify a new feasible solution for the DBLP using a local search on the solution identified in the previous step.
These solutions are found by assessing feasible `swaps' where we remove a selected drop box location from the tour and add a drop box location that is not visited by the incumbent tour.
Starting from a feasible solution, performing a feasible swap also results in a feasible solution.
As more iterations are completed, the identified solutions are required to provide an improved minimal access function value. 
% In the second step, we find multiple feasible solutions to the DBLP modifying the previous drop box locations in a local-search manner starting with the solution found in the first step.
% first step .
% A swap is only considered if the selected drop box locations would still satisfy all constraints in constraint set \eqref{model:basecoverage}.
% In each iteration, we progressively tighten a bound on to find solutions with increasing importance of the second objective.
Among the collection of solutions found, we discard the dominated solutions.

We describe the first step in more detail in Section \ref{sec:heuristicfirst} and describe the second step in more detail in Section \ref{sec:heuristicsecond}. 
% In Appendix \ref{sec:heuristicjustify} we provide a justification for the feasibility of the solutions found.
For ease, we make use of the reformulation of the first objective, $z_1$, described in Section \ref{sec:obj1reform}. % when introducing the heuristic.

While this heuristic algorithm is designed for the DBLP, it can also be used for similar problems in which the access function constraint set \eqref{model:obj2} takes a different form.
% used for other variants of the second objective, $z_2$. 
One variant of interest may be to measure the average access function \eqref{fun:coverage} value, rather than the minimum access function \eqref{fun:coverage} value. 
% , it may be desired to maximize the weighted average of the access function across all populations. 
% While the objective becomes non-linear with no straightforward linear equivalent, t
The heuristic method presented here can be easily adapted to this alternative objective.


\subsection{Step 1: Finding an Initial Solution}\label{sec:heuristicfirst}
In the first step of the heurstic method, we find a feasible solution to the DBLP of roughly minimal cost, $z_1$. 
Consider the following relaxation of the DBLP obtained from ignoring constraint set \eqref{model:obj2} and changing the right hand side of constraint set \eqref{model:basecoverage} from two to one. The relaxed integer program is:
%
\begin{align}
    \underset{x,y}{\min} \ &  \sum_{(i,j) \in E} \hat{c}_{ij} x_{ij}   \label{modelctp:obj}\\
    \text{s.t.} \ 
    & \sum_{i \in N_w} y_i \geq 1 & \forall \ w \in W \label{modelctp:basecoverage}\\
    &  \eqref{model:existing}, \eqref{model:balance} - \eqref{model:ybin} 
\end{align}
%
This relaxation is equivalent to the CTP \cite{gendreau_covering_1997}. We exploit this substructure of our problem to find an initial, feasible solution to the DBLP.
% We introduce the CTP in more detail before describing the procedure by which to identify an initial solution to the DBLP.
% to find a near-optimal initial solution to the DBLP of near-minimal cost.

% In the CTP, we are given an undirected weighted  graph $G = (H \cup M, A)$.
% % where $A = \{(i,j)\ |\ i,\ j \in V , \ i\neq j\}$ and the non-negative length of each edge is $c_{ij}$ (same as in DBLP).
% The nodes $H$ are the tour nodes and the nodes $M$ are the coverage nodes. 
% The objective of the CTP is to identify a tour visiting a subset of nodes 
% The subset of nodes $Y \subseteq M$ must be visited by the tour. Any node in $M \setminus Y$ can be visited but is not required to be.
% A node $h \in H$ is said to cover the nodes $M_h$ while a node $m \in M$ is covered by the nodes $H_m$.
% % In some cases, it is assumed that these sets are defined by some distance radius. In this paper, we deal with the general case of arbitrary covering sets.
% The objective of the CTP is to find a minimum length tour on the graph $G$ visiting a subset of nodes $H$ such that every vertex of $M$ is covered by at least one node visited by the tour. 

% We find an initial solution using a heuristic method to solve the covering tour problem (any heuristic method can be used, as desired). 
First, find a solution to the CTP instance using a heuristic or exact solution method.
Let $\hat{y}$ represent the drop box locations selected.
We construct a second CTP instance based on $\hat{y}$. For reference, we define $\hat{W}_2 \subset W$ as the voter populations for which $\hat{y}$ contains two elements of the coverage set, $|N_w \cap \hat{y}| \geq 2$.
We also let $\hat{T} : = T\cup \hat{y}$ be the union of $T$ and $\hat{y}$.
The second CTP instance is:
\begin{align}
    \underset{x,y}{\min} \ &  \sum_{(i,j) \in E} \hat{c}_{ij} x_{ij}   \label{modelctp:obj}\\
    \text{s.t.} \ 
    & y_t = 1 & \forall \ t \in \hat{T} \label{modelctp:existing} \\
    & \sum_{i \in N_w \setminus \hat{T}} y_i \geq 1 & \forall \ w \in W\setminus \hat{W}_2 \label{modelctp2:basecoverage}\\
    % & \sum_{i \in N : i,j \in E} x_{ij} = 2y_j & \forall \ j \in N \label{modelctp:balance} \\
    & \sum_{i \in S, j \in V\setminus S}    x_{ij} \geq 2y_t  & \forall \ S \subset V, \ 2 \leq |S| \leq |N|-2, \ \hat{T}\setminus S \neq \emptyset, t \in S \label{modelctp:subtourelim} \\
    % & x_{ij} \in \{0,1\} & \forall \ i \in N, j \in N \label{modelctp:xbin} \\
    % & y_{n} \in \{0,1\} & \forall \ n \in N \label{modelctp:ybin}
    & \eqref{model:balance}, \eqref{model:xbin}, \eqref{model:ybin}
\end{align}

Find a solution to the second CTP instance using a heuristic or exact solution method for the CTP.
This solution is feasible for the DBLP. This formally stated in Claim \ref{claim:hstep1}.
% Appendix \ref{sec:heuristicjustify} provides a justification for this claim.
% Solutions for the two CTP instances can be found using . 
The heuristic method we implement for the CTP is described in Appendix \ref{app:ctpheuristic}, but  any heuristic, approximate, or exact solution method for the CTP can be used.
% , but the steps do not rely on this specific implementation.
If a polynomial time heuristic method for the DBLP is desired, then the solution method for the CTP should also run in polynomial time.


\begin{claim}\label{claim:hstep1}
The tour found in Step 1 is feasible to the DBLP.
\end{claim}

% First, find a solution to the CTP instance as described by the relaxation to the DBLP above. 
% % By letting $H_1 := N$, $M_1 := W$, and $Y_1 := T$. We let the coverage sets for the CTP be naturally defined from $V_w$ and $W_v$.
% Let $H^*$ be the drop boxes selected to be included within the tour. 
% We construct a second instance to the CTP. 
% In this instance, we let $H := N$, $Y := T \cup H^*$, and $M := W\setminus \{w \in W\ :\ |V_w \cap H^*| \geq 2\}$ (i.e., voter locations covered at least twice by the drop boxes $H^*$). We let the coverage sets for the CTP be naturally defined from $V_w$, \emph{except} we remove the members of $Y$ from all coverage sets $V_w$.
% This is equivalent to defining $M_h = \emptyset$ for each $h \in Y$.
% We then find a solution to the CTP for this instance.
% The solution defines a feasible solution to to DBLP of near minimal cost.
% We let this solution be the in initial solution in our heuristic algorithm.



% We begin by describing the method by which to generate a feasible solution to the DBLP of (roughly) minimal cost.
% Consider the constraint  $\sum_{i \in N^{'}_w} y_i \geq 1$ for each $w \in W$ which is a relaxation of constraint set \eqref{model:basecoverage}.
% This constraint along with first objective $z_1$ and the constraint sets  \eqref{model:existing}, \eqref{model:balance}, \eqref{model:subtourelim}, \eqref{model:xbin}, \eqref{model:ybin}. 
% These together define an instance to the covering tour problem \cite{gendreau_covering_1997}.
% We exploit this fact. 

% First, find a solution for the covering tour instance using any available exact or heuristic method \cite{gendreau_covering_1997,alinaghian_two_2015,kubik_heuristic_2007,baldacci_scatter_2005,murakami_generalized_2018,vargas_dynamic_2017}. 
% Let $\hat{N} \subset N$ be the nodes of $N$ included within the solution to the covering tour problem. 
% Construct a second instance to the covering tour problem that is equivalent to the first except for the following three changes:
% \begin{enumerate}
%     \item Remove any $w \in W$ that is covered at least twice by $\hat{N}$.
%     \item Include all of $\hat{N}$ within the required nodes to visit.
%     \item Remove the members of \hat{N} from each coverage set.
% \end{enumerate}
% Solve this second instance to the covering tour problem. The solution is guaranteed to be feasible to the DBLP with (roughly) minimal cost. A local search procedure can be run to improve the cost if desired. Denote the nodes included within this tour as $N^0$.
% \textcolor{red}{Here we want to run some local search to improve the objective (allows for good solution to the variant). Ensure a feasible solution without improvement to the participation. Select cheapest swaps and until cant improve cost any more.}

% Do we want to use our Steiner Tree approach? \textcolor{red}{THIS IDEA WORKS FOR ANY SOLUTION TO THE COVERING TOUR PROBLEM} First generate Steiner Tree on auxiliary graph. Any node $v \in V$ spanned by the tree becomes 'required' (a part of $T$). Any node of W that is given double coverage by this tree is removed from the auxiliary graph. The edges incident to the nodes in the updated $T$ and members of $W$ are removed. If there are members of the updated $W$ that are not connected to the rest of the graph, the problem instance must be infeasible. On the updated auxiliary graph, we find a new Steiner Tree (approximate). This tree must span a subset of $N$ that provides double coverage to the set $W$. We then find a tour on this subset of nodes (using GENIUS? or exact?). \textcolor{red}{Could theoretically just start with a random set of nodes and keep running the procedure with no limit on worst case participation to then find a feasible solution...might node be any faster. Would need to make sure that the 'random' set provides double coverage}

\subsection{Step 2: Local Search} \label{sec:heuristicsecond}
Let $\mathcal{C}_{0}$ be the feasible tour identified in Step 1.
Let $N_{0}$ be the selected drop box locations. %$\mathcal{C}_{0}$.
Let $\alpha_{w,0} := v^0_{w}+v^1_{w}+\sum_{n \in N_{0}} v_{nw}$ be equal to the denominator of the access for $w\in W$ when drop boxes $N_{0}$ are added to the voting system.
Let $p_{w,0} := (\alpha_{w,0}-v^0_{w}) / \alpha_{w,0}$ represent the value of the access function for $w\in W$. 
% Also, let $I_{w,0} := |V_w \cap N_{0} |$ represent the number of nodes in $N_{0}$ that cover $w \in W$.


The remainder of the Step 2 progresses in an iterative fashion.
Let $k = 1,2,3,\dots$ represent the current iteration of the local search procedure. 
Let $\mathcal{C}_{k-1}$ be the tour identified by the previous iteration, and let $N_{k-1}$ be selected drop box locations.
The procedure is terminated once $N_{k-1} = N$.
Let $p_{w,k-1}$ represent the value of the access function for each $w \in W$ when drop boxes are placed at locations $N_{k-1}$.
Let $\alpha_{w,k-1}$ represent the value of the denominator of the access function.


Let $r_{k} :=  \min \{r_{k-1} + \varepsilon,\  \min_{w \in W} p_{w,k-1} \}$ represent the minimal allowable value of the access function for the solution output by after the $k^\text{th}$ iteration.
We initialize $r_0 := 0$.
The parameter $\varepsilon > 0$ is value, usually close to zero, provided as an input to limit the change between $r_{k-1}$ and $r_k$.
We define $r_{k}$ in this way to allow for solution \emph{back-tracking}.
Back-tracking occurs when the drop box locations defined by $N_{k-1}$ results in a substantially improved minimal access function value when compared to $N_{k-2}$ at the cost of a substantial increase in $z_1$.
% in an iteration, an added drop box may provide a substantial increase in the coverage of locations but with a large cost.
Back-tracking allows us to identify a new solution $N_k$ that substantially reduce the cost of the tour when compared to $N_{k-1}$ while still meeting a (slightly) tighter bound $r_k$. 



% That is, the collection of drop boxes, $N_k$ must satisfy
% $$r_k \geq \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{n \in N_k} v_{nw}} \quad \forall \ w \in W$$
% We assume a parameter $\varepsilon > 0$ with value close to zero is provided as an input to chap the change between $r_{k-1}$ and $r_k$.
% In the first iteration, we let $r_0 = 1$ and $r_k$ is updated at the end of the iteration. 

%
% Moreover, the collection of drop boxes is guaranteed to be feasible. Namely, $N_k$ must cover each population in $W$ twice. That is,
% $$ \sum_{i \in N_w \cap N_k} y_i \geq 2 \quad \forall \ w \in W $$
% The collections of $N_k \subseteq N$ that satisfy both these constraints are feasible for the DBLP in iteration $k$. 

In iteration $k$, we seek to identify a collection of drop box location $N_k$ and a tour $\mathcal{C}_{k}$ visiting these location that are feasible for the DBLP such that $z_2 \leq r_k$. 
However, determining the the $N_k$ and $\mathcal{C}_{k}$ that minimizes $z_1$ is NP-Hard. 
%
Instead, we take a local-search approach using the previous set of drop box location $N_{k-1}$.
% To identify feasible a collection of $N_k$ and $\mathcal{C}_{k}$ of roughly minimal cost, we consider a local-search from $N_{k-1}$.
% Thus, our heuristic method considers only incremental changes to $\mathcal{C}_{k-1}$ and $N_{k-1}$. Namely, we consider removing a drop box in $N_{k-1}$ from our system and adding a drop box not in $N_{k-1}$ to the system.
We define the neighborhood of solutions from $N_{k-1}$ as the collection of \emph{feasible swaps}.
A \emph{swap} is defined by two drop box locations $n_1$ and $n_2$ with the prior indicating a drop box location to remove from the incumbent solution and the later indicating a drop box location to add to the incumbent solution ($n_1$, $n_2$ can also represent ``no drop box location''). 
There are $\mathcal{O}(|N|^2)$ swaps.
A swap is feasible if starting with a feasible set of drop box locations $N_{k-1}$, the following two conditions hold:
$$r_{k}  \leq \frac{v^1_{w}+\sum_{n \in N_{k-1}\setminus \{n_1\}\cup\{n_2\}} v_{nw} }{v^0_{w}+v^1_{w}+\sum_{n \in N_{k-1}\setminus \{n_1\}\cup\{n_2\}} v_{nw} } \quad  \forall \ w\in W$$
% $$ \sum_{n \in N_w} \mathbbm{1}(n \in N_{k-1}\setminus \{n_1\}\cup\{n_2\}) \geq 2 \quad  \forall \ w\in W$$
$$ | \{n \in N_w : n \in N_{k-1}\setminus \{n_1\}\cup\{n_2\}\} | \geq 2 \quad  \forall \ w\in W$$
The first condition ensures that the minimum access function value is at least $r_k$.
The second condition ensures that the selected drop box locations satisfy constraint set \eqref{model:basecoverage}.
These can be verified in polynomial time.
In the cases in which $n_1$ or $n_2$ represent ``no drop box location'', $v_{n_\cdot,w} = 0$.
In Appendix \ref{app:heuristic}, we describe a scheme that reduces the number of operations that must be performed to verify if a swap is feasible.


% In the cases in which $n_1$ and $n_2$ represent ``no drop box location'', $v_{n_\cdot,w} = 0$ and $W_{n_\cdot} = \emptyset$ for the `no drop box'.

% A tour over the updated nodes is later found. We call this a `swap'.
% We can check the feasibility of a swap as follows. 
% Let $n_1$ be a potential drop box to remove and $n_2$ a potential drop box to add. 
% For the swap of $n_1$ for $n_2$ to be feasible in iteration $k$, we verify the following two statements hold
% % We can check if $n_1$ and $n_2$ define a feasible swap by checking the following two statements.
% $$ r_{k}  \geq \max_{w \in W}{\ p_{w,k-1}+ v^0_{w}(v_{n_1w} - v_{n_2w}) / (\alpha_{w,k-1}*(\alpha_{w,k-1} - v_{w,n_1} + v_{n_2w}))} $$
% $$\{w \in W_{n_1} : I_{w,k-1} = 2\} \subseteq W_{n_2}$$

Each feasible swap will result in an updated cost value, $z_1$, and updated minimum access function value. 
We refer to the minimum access function value as $z_2$.
Let $\Delta z_1$ represent the difference in the cost of the tour $\mathcal{C}_{k-1}$ and a tour over $N_{k-1}\setminus \{n_1\}\cup\{n_2\}$.
Rather than finding the optimal tour over $N_{k-1}\setminus \{n_1\}\cup\{n_2\}$, which is NP-Hard, we estimate $\Delta z_1$ by removing $n_1$ from $\mathcal{C}_{k-1}$ and finding the lowest cost insertion of $n_2$ into this updated tour. % into $\mathcal{C}_{k-1}\setminus \{n_1\}$.
If $r_{k} = r_{k-1}-\varepsilon$, a swap with an $\Delta z_1 > 0$ is considered infeasible. This leads to lower cost solutions when possible.
Let $\Delta z_2$ represent the difference in $z_2$ when using drop box locations $N_{k-1}\setminus \{n_1\}\cup\{n_2\}$ compared to $N_{k-1}$.
We let the \emph{value} of a swap be equal to $\Delta z_1/\Delta z_2$.
Among all feasible swaps, we select the one with the highest value.
The feasible swap with the highest value is the \emph{selected swap}.

Given the selected swap, we build the new feasible solution for the DBLP and update the parameters.
% Once we identify the optimal swap, we must update our parameters. 
Let $n_1$ represent the drop box to remove from the tour and let $n_2$ represent the drop box to add to the tour. 
The new feasible set of drop box location $N_k$ and parameter value are:
$$N_{k} = N_{k-1} \cup \{n_2\} \setminus \{n_1\}$$
$$\alpha_{w,k} = \alpha_{w,k-1}- v_{n_1w}+v_{n_2w} \quad \forall \ w \in W $$
% $$p_{w,k} = p_{w,k-1}+v^0_{w}(v_{n_1w} -v_{n_2w}) / (\alpha_{w,k-1}*\alpha_{w,k}) \quad \forall \ w \in W$$
$$p_{w,k} = (\alpha_{w,k} - v^0_{w})/ \alpha_{w,k} \quad \forall \ w \in W$$
A tour $\mathcal{C}_k$ over $N_k$ can be found in polynomial time using any polynomial time TSP heuristic such as the GENIUS algorithm \cite{gendreau_new_1992}.
In our implementation, we elect to solve the TSP to optimality over $N_k$ as the number of drop box locations selected is relatively small and solutions can be found quickly once the drop box locations are known.

Once the iterative procedure is terminated, return all non-dominated solutions among $N_k$, $\mathcal{C}_k$ for $k \in \{1,2,3,\dots\}$. 
To do so, disregard solutions that have both a worse $z_1$ and worse minimal access function value than another solution found by the heuristic.




\subsection{Heuristic Results}
Despite the combinatorial challenges posed by our problem, we find that our proposed heuristic method approximates the Pareto frontier between cost and the minimum access function value well and does so quickly.
Figure \ref{fig:frontier_compare} plots the cost and minimum access function of policies found using the exact method (\ref{fig:frontier_exact}) against the policies found using the heuristic method (\ref{fig:frontier_heuristic}) for four instances of the case study, each corresponding to coverage sets defined by a different factor (1.0, 1.1, 1.2, or 1.3).
% Other instances of the problem produce similar plots.
Computational studies were run on using 64 bit Python 3.7.7 on an Intel\textsuperscript{\textregistered} Core\textsuperscript{TM} i5-7500 CPU with 16 GB of RAM. The exact solution method was implemented using Gurobi 9.1.
\textcolor{red}{Out implementation of the heuristic uses the approach in Appendix X to find a solution to the CTP and solves the TSP to optimiality (rather than using a heuristic) when a collection of locations are selected as it solves quickly.}
% 12788.9369141 seconds
We find that the the exact method can find a new policy every 225 seconds on average. 
The heuristic method presented in Section \ref{sec:heuristic} is able to generate between 88-114 policies in 84-120 seconds depending on the factor.
\textcolor{red}{Since the solution method to the CTP has some randomness, the heuristic method can be rerun multiple times.
The non-dominated solutions among all runs can be kept.
Experiments show that this can improve how well the heuristic method matches the exact method.
}
% We find that instances corresponding to larger coverage sets (larger factor) require longer  
% cause solution times substantially increase using the exact method (in some cases $>4$ hours for a single solution) while the heuristic method remains relatively unchanged ($\leq 150$ seconds for the compete frontier).
% , solution times quickly increase and some solutions take longer than two hours to find. 
A primary benefit of our proposed heuristic method is to highlight the trade-off between the minimum access function value and the cost of the drop box system ($z_1$) so that election officials can determine an appropriate location on the frontier to find an optimal solutions.
Once an appropriate location on the Pareto frontier is selected, the optimal solution at that location of the Pareto frontier can be found using the exact solution.
% However, as noted earlier, even a single solution can take multiple hours to find.

% at that location can be solved relatively quickly. On average, the optimal solution can be found in approximately 10 minutes on average once the minimal allowable value for the access function is known.


% \begin{figure}[H]%[!htb]
% \centering
% \captionsetup{width = 0.9\textwidth}
% \begin{tikzpicture}
% \begin{axis}[
% 	width=0.7\textwidth,
%       height=0.4\textwidth,
%       axis lines=middle,
%       legend columns = 2,
%       scaled y ticks=false,
%         legend style={at={(0.5,-0.38)},anchor=south},
%         legend cell align={left},
%         x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
%         y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
%         ylabel={Cost ($z_1$)},
%         yticklabel style={
%         /pgf/number format/fixed,
%         /pgf/number format/precision=5
%         },
%         xlabel={Minimum access function value},
%         enlargelimits = true,
%         legend columns = 3,
%         % ymin = 150,
%         % ymax= 500,
%         % xmin = 0.4.
%         % xmax = 0.7
%           ] 
%       \addplot[mark=triangle,black] table [y=C,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Exact Method} \label{fig:frontier_exact}
%       \addplot[const plot mark right,red] table [y=C_1.0,x=P_1.0, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic Method} \label{fig:frontier_heuristic}
%       %
%       %% These are the rules-of-thumb for comparison
%     %   \addplot[mark size=2pt,mark options={color=blue}, only marks] plot coordinates {(0.542119954600902,2601.676216)
%     %     (0.557504137420686,11099.9264514)
%     %     (0.568047601927534,21015.6370626667)
%     %     (0.581764939515681,25154.43166572)
%     %     (0.590925741698136,31394.7444396)
%     %     (0.622864340093998,46328.5055448666)
%     %     (0.559995693279841,20299.5882997999)
%     %     }; 
%  \end{axis}
% \end{tikzpicture}
% \caption{\centering Approximate Pareto frontier identified by the heuristic method compared to the exact solution method. } \label{fig:frontier_compare}
% \end{figure}


\begin{figure}[H] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \begin{tikzpicture}
\begin{axis}[
	width=0.95\textwidth,
      height=0.7\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.02,0.98)},anchor=north west},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        ylabel={Cost ($z_1$)},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={Minimum access function value},
        enlargelimits = true,
        legend columns = 1,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Exact} \label{fig:frontier_exact}
      \addplot[const plot mark right,red] table [y=C_1.0,x=P_1.0, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic} \label{fig:frontier_heuristic}
      \addplot[const plot mark right,orange] table [y=C_1.0,x=P_1.0, col sep=comma]{frontier_heuristic_mke2.csv};
      %
    %   % These are the rules-of-thumb for comparison
    %   \addplot[mark size=2pt,mark options={color=blue}, only marks] plot coordinates {(0.542119954600902,2601.676216)
    %     (0.557504137420686,11099.9264514)
    %     (0.568047601927534,21015.6370626667)
    %     (0.581764939515681,25154.43166572)
    %     (0.590925741698136,31394.7444396)
    %     (0.622864340093998,46328.5055448666)
    %     (0.559995693279841,20299.5882997999)
    %     }; 
 \end{axis}
\end{tikzpicture} 
    \caption{Factor of 1.0} 
    \label{fig7:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \begin{tikzpicture}
\begin{axis}[
	width=0.95\textwidth,
      height=0.7\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.5,-0.38)},anchor=south},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        ylabel={Cost ($z_1$)},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={Minimum access function value},
        enlargelimits = true,
        legend columns = 3,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C_1.1,x=P_1.1, col sep=comma]{frontier_equality.csv};\addlegendentry{Exact Method} \label{fig:frontier_exact}
      \addplot[const plot mark right,red] table [y=C_1.1,x=P_1.1, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic Method} \label{fig:frontier_heuristic}
      \addplot[const plot mark right,orange] table [y=C_1.1,x=P_1.1, col sep=comma]{frontier_heuristic_mke2.csv};
      \legend{}; % empty the legend so as not to print it
      %
    %   % These are the rules-of-thumb for comparison
    %   \addplot[mark size=2pt,mark options={color=blue}, only marks] plot coordinates {(0.542119954600902,2601.676216)
    %     (0.557504137420686,11099.9264514)
    %     (0.568047601927534,21015.6370626667)
    %     (0.581764939515681,25154.43166572)
    %     (0.590925741698136,31394.7444396)
    %     (0.622864340093998,46328.5055448666)
    %     (0.559995693279841,20299.5882997999)
    %     }; 
 \end{axis}
\end{tikzpicture}
    \caption{Factor 1.1} 
    \label{fig7:b} 
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \begin{tikzpicture}
\begin{axis}[
	width=0.95\textwidth,
       height=0.7\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.5,-0.38)},anchor=south},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        ylabel={Cost ($z_1$)},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={Minimum access function value},
        enlargelimits = true,
        legend columns = 3,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C_1.2,x=P_1.2, col sep=comma]{frontier_equality.csv};\addlegendentry{Exact Method} \label{fig:frontier_exact}
      \addplot[const plot mark right,red] table [y=C_1.2,x=P_1.3, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic Method} \label{fig:frontier_heuristic}
      \addplot[const plot mark right,orange] table [y=C_1.2,x=P_1.2, col sep=comma]{frontier_heuristic_mke2.csv};
      \legend{}; % empty the legend so as not to print it
      %
    %   % These are the rules-of-thumb for comparison
    %   \addplot[mark size=2pt,mark options={color=blue}, only marks] plot coordinates {(0.542119954600902,2601.676216)
    %     (0.557504137420686,11099.9264514)
    %     (0.568047601927534,21015.6370626667)
    %     (0.581764939515681,25154.43166572)
    %     (0.590925741698136,31394.7444396)
    %     (0.622864340093998,46328.5055448666)
    %     (0.559995693279841,20299.5882997999)
    %     }; 
 \end{axis}
\end{tikzpicture} 
    \caption{Factor 1.2} 
    \label{fig7:c} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \begin{tikzpicture}
\begin{axis}[
	width=0.95\textwidth,
      height=0.7\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.5,-0.38)},anchor=south},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        ylabel={Cost ($z_1$)},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={Minimum access function value},
        enlargelimits = true,
        legend columns = 3,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C_1.3,x=P_1.3, col sep=comma]{frontier_equality.csv};\addlegendentry{Exact Method} \label{fig:frontier_exact}
      \addplot[const plot mark right,red] table [y=C_1.3,x=P_1.3, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic Method} \label{fig:frontier_heuristic}
      \addplot[const plot mark right,orange] table [y=C_1.3,x=P_1.3, col sep=comma]{frontier_heuristic_mke2.csv};
      \legend{}; % empty the legend so as not to print it
      %
    %   % These are the rules-of-thumb for comparison
    %   \addplot[mark size=2pt,mark options={color=blue}, only marks] plot coordinates {(0.542119954600902,2601.676216)
    %     (0.557504137420686,11099.9264514)
    %     (0.568047601927534,21015.6370626667)
    %     (0.581764939515681,25154.43166572)
    %     (0.590925741698136,31394.7444396)
    %     (0.622864340093998,46328.5055448666)
    %     (0.559995693279841,20299.5882997999)
    %     }; 
 \end{axis}
\end{tikzpicture}
    \caption{Factor 1.4} 
    \label{fig7:d} 
  \end{subfigure} 
  \caption{\centering Approximate Pareto frontier identified by the heuristic method compared to the exact solution method. } \label{fig:frontier_compare}
\end{figure}


\subsection{Covering Tour Problem Heuristic}\label{app:ctpheuristic}
Let $G$ be a graph for the CTP defined by node sets $H,\ M$, and $Y$ and edges $A$.
We construct an auxiliary graph.
Let $G' = (R \cup S, \hat{A})$ be the undirected weighted auxiliary graph.
Let $R = Y \cup M$ and $S = H\setminus Y$.
%
Let $\hat{A} = A \cup \{(h,m)\ |\ h \in H,\ m \in M_h\}$ a set of weighted edges. The first subset of edges ($A$) are the edges in the graph $G$. 
The second subset are edges incident to a node $h \in H$ and a node $m \in M_h$ that it covers in the CTP. 
%
We defined the length of each edge in $\hat{A}$ as follows. Let the length of edges in $A$ be the same as that in $G$. Let $K = \max_{(i, j) \in A} \{ c_{ij} \}$ be the maximum length edge in $A$. Let the length of each edge $(h,m)$ for $m \in M$ and $h \in H_m$ be $\frac{K(|H|-1)}{|H|+|M|-1}$.

On this graph, find a heuristic solution for the Steiner tree problem with Steiner nodes $S$ and required nodes $R$ using the SketchLS heuristic introduced by \citet{gubichev_fast_2012}.
Of the nodes spanned by the tree, identify those belonging to $H$. Denote these nodes as $H^*$.
This set of nodes may contain nodes that provide no marginal value to the coverage of nodes in $M$. 
Iteratively remove nodes from $H^* \setminus T$ that provide no marginal coverage.
We check nodes in the order of size of $M_h$ (largest first).
Then find and return a tour on the resulting $H^*$.
This can be done using a heuristic for the TSP, such as the GENIUS algorithm \cite{gendreau_new_1992} or an exact method. In our implementation, we solve the tour to optimality using lazy constraints.



\subsection{Alternative Feasibility Check for Heuristic Solution Method}\label{app:heuristic}
% We prove the feasibility of the solution output after each iteration inductively. 
% We begin with the selection of drop boxes defined by $N_0$.
% We need only consider constraint set \eqref{model:basecoverage} to verify feasibility, assuming that the CTP heuristic algorithm used indeed returns a valid tour over the selected nodes.
% Recall the procedure introduced in Section \ref{sec:heuristicfirst}.
% Suppose $N_0$ is not feasible to the RDBP. 
% Then $N_0$ does not satisfy the constraint set \eqref{model:basecoverage}.
% Then for some $w \in W$, it is true that $\sum_{i \in N_w} \mathbbm{1}[n \in N_0] = |N_w \cap N_0| < 2$. 
% Thus, $|N_w \cap N_0|$ is either zero or one. 
% Consider the case where $|N_w \cap N_0|=0$. Then $|N_w \cap \hat{T}| = 0$ which implies $|N_w \cap \hat{y}| = 0$. This contradicts the fact that $\hat{y}$ defines the nodes of a feasible CTP solution to the first instance solved.
% Consider the case where $|N_w \cap N_0|=1$. 
% Recall in the second CTP instance,  $\hat{T}$ defines a collection of nodes that collectively cover every $w \in W$ at least once as $\hat{T} = T \cup \hat{y}$.
% In addition, in the second CTP instance, the coverage set in \eqref{modelctp:basecoverage} for each $w \in W$ contains no drop box location within $\hat{T}$. 
% Thus, it must be true that $|N_w \cap N_0|=1+|N_w \cap N_0\setminus \hat{T}|$. Thus, $|N_w \cap N_0\setminus Y| = 0$. However, this contradicts the fact that we have a feasible solution to the second CTP instance.
% Thus, the initial solution found by our heuristic algorithm must be feasible to the DBLP.

% We argue that the procedure will result in a set of nodes $N_0$ from which each $w \in W$ is covered twice. 
% Suppose this is not the case. Then with $w$ is covered zero or one times.
% The initial solution to the CTP ensures that each $w$ is covered at least once. The set of nodes providing this single coverage are then added to the set of required nodes in the second solution generation. 
% Suppose after the second solution, there is a $w$ that is only covered once. We argue this is not possible. We must only focus on the $w$ for which the coverage was one after the first solution generation. All other $w$ must be covered at least twice by the required nodes of the second generation.
% For each of these $w$, we remove the required nodes from their coverage set and resolve. Thus, we identify a second node that covers $w$.
% The resulting nodes must cover each $w$ twice.

Let $W_{n} \subseteq W$ represents the voter populations $w\in W$ for which $n\in N$ is a member of $N_w$, $W_{n} := \{w \in W: n \in N_w \}$. These sets can be precomputed in polynomial time.
Let $I_{w,k-1} := |V_w \cap N_{k-1} |$ represent the number of nodes in $N_{k-1}$ that cover $w \in W$ in iteration $I_{k-1}$.
Let $I_{w,0}$ be initialized based on $N_0$.

Given $N_{k-1}$, we can verify if a pair $(n_1,n_2)$ represents a feasible swap by checking the following conditions:
% $$ r_{k}  \geq p_{w,k-1}+ v^0_{w}(v_{n_1w} - v_{n_2w}) / (\alpha_{w,k-1}*(\alpha_{w,k-1} - v_{w,n_1} + v_{n_2w}))  \quad  \forall \ w\in W$$
$$v^0_{w} \leq (1-r_k) (\alpha_{w,k-1} -v_{n_1 w} +v_{n_2 w}) \quad \forall \ w\in W$$
$$\{w \in W_{n_1} : I_{w,k-1} = 2\} \subseteq W_{n_2}$$


Moreover, the following provides the correct value of $I_{w,k}$ given the selected swap $n_1$ and $n_2$ if $I_{w,k-1}$ is correct.
$$I_{w,k} = \begin{cases}
      I_{w, k-1} - 1  &  \text{if }w \in W_{n_1} \setminus W_{n_2} \\
      I_{w, k-1} +1 &  \text{if } w \in W_{n_2} \setminus W_{n_1}\\
      I_{w, k-1}  & \text{otherwise}
    \end{cases} \quad \forall \ w \in W$$

We next show the parameters retain the correct definition throughout the solution method. 
Note that we begin with $I_{w,0} = |V_w \cap N_{0}|$ for each $w \in W$. By induction, in iteration $k$:
% After finding the initial solution, we compute the parameters $p_{w,0}$, $\alpha_{w,0}$, and $I_{w,0}$ exactly.
% Suppose we are given $\alpha_{w,k-1}$, $p_{w,k-1}$, and $I_{w,k-1}$ where $\alpha_{w,k-1}$ represents the denominator of the access function for population $w\in W$ given drop box location $N_{k-1}$, $p_{w,k-1}$ is the value of the access function for population $w\in W$, and $I_{w,k-1}$ represents the number of drop boxes in $N_{k-1}$ that are also in $N_w$ for population $w \in W$.
% We show that our updating procedure yield value of $\alpha_{w,k}$, $p_{w,k}$, and $I_{w,k}$ such that they equal the following terms:
% \begin{align}
%     \alpha_{w,k} & = v^0_{w}+v^1_{w}+\sum_{j \in N_{k}} v_{jw} \nonumber \\
%     p_{w,k} & = \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N_{k}} v_{jw}} \nonumber \\
%     I_{w,k} & = |N_{k}\cap N_w| \nonumber 
% \end{align}

% We begin with $\alpha_{w,k}$.
% \begin{align}
%     \alpha_{w,k} & = \alpha_{w,k-1} - v_{n_1w}+v_{n_2w}  \nonumber \\
%     & = v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw} - v_{n_1w}+v_{n_2w}  \nonumber \\
%     & = v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}\cup\{n_2\}\setminus\{n_1\}} v_{jw}  \nonumber \\
%     & = v^0_{w}+v^1_{w}+\sum_{j \in N_{k}} v_{jw}  \nonumber 
% \end{align}
%
% Next, we show that the statement is true for $p_{w,k}$.
% \begin{align}
%      p_{w,k} & = p_{w,k-1}+\frac{v^0_{w}(v_{n_1w} -v_{n_2w})}{ \alpha_{w,k-1}\alpha_{w,k}} \nonumber \\
%      & = \frac{v^0_{w}}{\alpha_{w,k-1}} +  \frac{v^0_{w}(v_{n_1w} -v_{n_2w})}{\alpha_{w,k-1}\alpha_{w,k}} \nonumber\\
%     %  & = \frac{v^0_{w}}{\alpha_{w,k-1}} + \frac{v^0_{w}(v_{n_1w} -v_{n_2w})}{\alpha_{w,k-1}*\alpha_{w,k}} \nonumber\\
%      & = \frac{v^0_{w}\alpha_{w,k}}{\alpha_{w,k-1}\alpha_{w,k}} + \frac{v^0_{w}(v_{n_1w} -v_{n_2w})}{\alpha_{w,k-1}\alpha_{w,k}} \nonumber\\
%      & = \frac{v^0_{w}(\alpha_{w,k-1} - v_{w,n_1} + v_{w,n_2})+v^0_{w}(v_{n_1w} -v_{n_2w})}{\alpha_{w,k-1}(\alpha_{w,k-1} - v_{w,n_1} + v_{w,n_2})} \nonumber\\
%      & = \frac{v^0_{w}(\alpha_{w,k-1} - v_{w,n_1} + v_{w,n_2}+v_{n_1w} -v_{n_2w})}{\alpha_{w,k-1}(\alpha_{w,k-1} - v_{w,n_1} + v_{w,n_2})} \nonumber\\
%      & = \frac{v^0_{w}\alpha_{w,k-1}}{\alpha_{w,k-1}(\alpha_{w,k-1} - v_{w,n_1} + v_{w,n_2})} \nonumber\\
%      & = \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw} - v_{w,n_1} + v_{w,n_2}} \nonumber \\
%     & = \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N_{k}} v_{jw}} \nonumber
% \end{align}
% Note that if $n_1$ or $n_2$ represent `no drop box', the parameter $v_{n_\cdot,w}$ equals zero.

% Lastly, we show that the statement is true for $I_{w,k}$. Note that if $n_1$ or $n_2$ represent `no drop box', the set $W_{n_\cdot} = \emptyset$.

% \textbf{Finding a valid swap - coverage feasibility!}
% First,  ensuring that the count in each iteration is correct. 
\begin{align}
    I_{w,k} &= \begin{cases}
      I_{w, k-1} - 1  &  \text{if }w \in W_{n_1} \setminus W_{n_2} \\
      I_{w, k-1} +1 &  \text{if } w \in W_{n_2} \setminus W_{n_1}\\
      I_{w, k-1}  & \text{otherwise}
    \end{cases} \nonumber \\
    &= \begin{cases}
      |N_{k-1}\cap N_w| - 1  &  \text{if } w \in W_{n_1} \setminus W_{n_2} \\
      |N_{k-1}\cap N_w| + 1 &  \text{if } w \in W_{n_2} \setminus W_{n_1}\\
      |N_{k-1}\cap N_w|  & \text{otherwise}
    \end{cases}  \nonumber \\
    % &= \begin{cases}
    %   |(N_{k-1}\setminus \{n_1\}) \cap N_w| &  \text{if } w \in W_{n_1} \setminus W_{n_2}  \\
    %   |(N_{k-1}\cup \{n_2\}) \cap N_w| &  \text{if } w \in W_{n_1} \setminus W_{n_2}  \\
    %   |(N_{k-1})\cup \{n_2\}\setminus \{n_1\} \cap N_w|  & \text{otherwise}
    % \end{cases}  \nonumber \\
    & = |(N_{k-1}\cup \{n_2\}\setminus \{n_1\}) \cap N_w| \nonumber \\
    &= |N_{k}\cap N_w| \nonumber 
\end{align}



Finally, we consider the feasibility of the solution output in the $k^\text{th}$ iteration:
\begin{align}
    &v^0_{w} \leq (1-r_k) (\alpha_{w,k-1} -v_{n_1 w} +v_{n_2 w}) & \forall \ w\in W \nonumber \\
    & \frac{v^0_{w}}{\alpha_{w,k-1} -v_{n_1 w} +v_{n_2 w}} \leq 1-r_k & \forall \ w\in W \nonumber \\
    & \frac{v^0_{w}}{v^0_{w} + v^1_{w} + \sum_{n \in N_{k-1}}v_{n w} -v_{n_1 w} +v_{n_2 w}} \leq 1-r_k & \forall \ w\in W \nonumber \\
    & \frac{v^0_{w}}{v^0_{w} + v^1_{w} + \sum_{n \in N_{k}}v_{n w}} \leq 1-r_k & \forall \ w\in W \nonumber \\
    &  r_k \leq 1-\frac{v^0_{w}}{v^0_{w} + v^1_{w} + \sum_{n \in N_{k}}v_{n w}} & \forall \ w\in W \nonumber \\
    &  r_k \leq \frac{v^1_{w} + \sum_{n \in N_{k}}v_{n w}}{v^0_{w} + v^1_{w} + \sum_{n \in N_{k}}v_{n w}} & \forall \ w\in W \nonumber
\end{align}
Now we must check that constraint set \eqref{model:basecoverage} is satisfied by $N_k$.
% We must verify the following double-coverage condition holds when we `swap' $n_1$ with $n_2$ to obtain $N_k$.
We have already shown that $I_{w,k}$ equals $|N_{k} \cap N_w|$ for each $w \in W$. Assume that $I_{w,k-1} \geq 2$; we show that $I_{w,k} \geq 2$ for each $w \in W$.
For each $w \in W$, there are three possibilities:
\begin{enumerate}
    \item $ w \in W_{n_2} \setminus W_{n_1}$: By construction $I_{w,k} = I_{w,k-1}+1 \geq 2$ since $I_{w,k-1} \geq 2$.
    \item $w \in W_{n_1} \setminus W_{n_2}$: By construction $I_{w,k} = I_{w,k-1} -1$. We have two cases: $I_{w,k-1} \geq 3$ or $I_{w,k-1} = 2$. 
    In the first case, $I_{w,k} = I_{w,k-1} -1 \geq 2$ since $I_{w,k-1} \geq 3$ and at most one location is removed.
    In the second, it must be true that $n_1$ and $n_2$ satisfy $\{w \in W_{n_1} : I_{w,k} = 2\} \subseteq W_{n_2}$. This implies a $w$ such that $w \in W_{n_1} \setminus W_{n_2}$ and $I_{w,k-1} = 2$ cannot exist.
% We now deal with the second case. Note that in each iteration, $I_{w,k} \geq I_{w,k} = I_{w,k-1} - 1 $ by construction. Thus $I_{w,k} \geq I_{w,k} - 1 \geq 3-1 \geq 2$. 
    \item All other cases: By construction $I_{w,k} = I_{w,k-1} \geq 2$.% since $I_{w,k-1} \geq 2$.
\end{enumerate}




% Then, determining the coverage of each node $w \in W$.
% We need to ensure that in each iteration $k$, we find a set of nodes $N_k$ that cover each $w \in W$ twice. That is $|N_k \cap N_w| \geq 2$ for each $w \in W$. 
% % We do so by verifying that $\{w \in W_{n_1} : I_{w,k} = 2\} & \subseteq W_{n_2}$.  
% In each iteration, we enforce that to remove $n_1$ and remove $n_2$, it must be true $\{w \in W_{n_1} : I_{w,k} = 2\} & \subseteq W_{n_2}$.
% We argue this is a sufficient condition to ensure $|N_k \cap N_w| \geq 2$.


% In the first iteration, we start with a set of nodes $N_{0}$ for which this condition is satisfied.
% Now assume that $N_{k-1}$ satisfies this condition. That is, $I_{w,k-1} = |N_k \cap N_w| \geq 2$ for each $w \in W$.
% We show that it must be true $I_{w,k} \geq 2$ for each $w \in W$.
% Suppose that this is not true and $w \in W$, $I_{w,k} < 2$.
% It must be true for $w$ that $I_{w,k}=2$ since we remove at most a single node from $N_{k-1}$/.
% Let $n_1$ and $n_2$ be the nodes removed and added in iteration $k$. 

% If $n_1 \not\in W_{n_2}$

% In the first iteration, we start with a set of nodes $N_{0}$ for $I_{w,0} = |N_0 \cap N_w| \geq 2$ for each $w \in W$.
% Now assume that in the $k-1^\text{th}$ iteration $I_{w,k-1} = |N_{k-1} \cap N_w| \geq 2$ for each $w \in W$.
% It is sufficient to show that $I_{w,k-1}\geq 2$ for each $w \in W$.
% Let $n_1$ and $n_2$ be the nodes removed and added, respectively, in iteration $k$. 
% We consider the three possibilities: 

% (1) $ w \in W_{n_2} \setminus W_{n_1}$: By construction $|N_0 \cap N_w| = I_{w,k} = I_{w,k-1}+1 \geq 2$ since $I_{w,k-1} \geq 2$.

% (2)  $w \in W_{n_1} \setminus W_{n_2}$: By construction $|N_0 \cap N_w| = I_{w,k} = I_{w,k-1} -1$. 
% We have two cases: $I_{w,k-1} = 2$ or $I_{w,k-1} \geq 3$. 
% We deal with the first case: It must be true that $n_1$ and $n_2$ satisfy $\{w \in W_{n_1} : I_{w,k} = 2\} \subseteq W_{n_2}$. This implies that there cannot be such a $w$.
% We now deal with the second case. Note that in each iteration, $I_{w,k} \geq I_{w,k} = I_{w,k-1} - 1 $ by construction. Thus $I_{w,k} \geq I_{w,k} - 1 \geq 3-1 \geq 2$. 

% (3) All other cases: By construction $|N_0 \cap N_w| = I_{w,k} = I_{w,k-1} \geq 2$ since $I_{w,k-1} \geq 2$.






% Let $k$ be the count of the current iteration of the procedure. Let $N_{k-1}$ be the nodes included within the previous tour. Let $p_{w, k-1}$ be the participation rate of node $w$ in the previous iteration. Let $r_{k-1}$ be the worst case participation rate after the previous iteration. At the beginning of the procedure, we can initialize $p_{w,0}$ for each $w \in W$ based on the participation when using the lowest tour cost solution. We must determine the participation rate given a swap of $n^1_{k}$ included in the $k-1^{\text{th}}$ tour and $n^2_{k}$ a node not included in the previous tour. In each iteration, we must improve the participation of the worst case voter by at least $\varepsilon$. That is, we must find a swapping of $n^1_{k}$ and $n^2_{k}$ that results in $r_k \leq r_{k-1} - \varepsilon$. \textcolor{red}{NOTE: $n^1$ can be a dummy representing no node.}

% The \textbf{change} in non-participation rate, $\Delta_{w n^1 n^2}$, of node $w$ given swap of $n^1$ with $n^2$ is:


% \begin{align}
%     \Delta_{w n^1 n^2} \ & = \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1} \setminus n^1  \cup n^2 } v_{jw}} - \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw}} \nonumber \\
%     \Delta_{w n^1 n^2}(v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1} \setminus n^1  \cup n^2 } v_{jw})(v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw}) \ & =   v^0_{w}(v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw}) -  v^0_{w}(v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1} \setminus n^1  \cup n^2 } v_{jw}) \nonumber \\
%     & =  v^0_{w}(v^0_{w}+v^1_{w}+\sum_{j \in N_{k-1}} v_{jw} - v^0_{w}  - v^1_{w} - \sum_{j \in N_{k-1} \setminus n^1  \cup n^2 } v_{jw}) \nonumber \\
%     & =  v^0_{w}(\sum_{j \in N_{k-1}} v_{jw} - \sum_{j \in N_{k-1} \setminus n^1  \cup n^2 } v_{jw}) \nonumber \\
%     & =  v^0_{w}(v_{n^1 w} - v_{n^2w}) \nonumber 
% \end{align}
% \textcolor{red}{Deal with the denominator}
% So then, the participation constraint set can be reformulated to be:
% $$ p_{w, k-1} +  v^0_{w}(v_{n^1 w} - v_{n^2w})/denom  \leq r_{k-1} - \varepsilon_k \quad \forall \ w \in W $$
% % \begin{align}
%     % \frac{v^1_{w}+\sum_{j \in N^* \setminus n \cup n^*} v_{jw} }{v^0_{w}+v^1_{w}+\sum_{j \in N^*\setminus n \cup n^*} v_{jw} } \leq r - \varepsilon \nonumber \\
% % \end{align}

% \textcolor{red}{Note that if among all added node (no removes) the resulting participation is not low enough for $\varepsilon$, we take add the node with the minimal worst case participation. This is done because in some cases, we may need to add two nodes to maintain feasibility and improve participation enough. We could always consider adding up to k of the added nodes without removing any (for large k however, this grows exponentially as it is n choose k.}


% Then there is an $n_1$ and $n_2$ for which $\{w \in W_{n_1} : I_{w,k} = 2\} & \subseteq W_{n_2}$, but that resulted in $N_k = N_{k-1} \cup \{n_2\} \setminus \{n_1\}$ for which $|N_k \cap N_w| < 2$ for some $w \in W$. 

% Note that $I_{w,k} \geq 2$ for each $w \in W$ and $k$.

% Then there must exist some $w \in W_{n_1}$ and $\in W_{n_2}$ for which $I_{w,k} \geq 2$. 
% Note that $w \not\in W_{n_1}\setminus W_{n_2}$ and $w \not\in W_{n_2}\setminus W_{n_1}$ since $w$ is in both $W_{n_1}$ and $W_{n_1}$.
% By construction of , $I_{w,k} = I_{w,k-1}-1$ in this case. 

% \begin{align}
%     \{w \in W_{n_1} : I_{w,k} = 2\} & \subseteq W_{n_2} \nonumber \\
%     \{w \in W_{n_1} : |N_{k}\cap N_w| = 2\} & \subseteq W_{n_2} \nonumber
% \end{align}

% We must ensure that a feasible swap results in a collection of nodes that provide double coverage to each node in $W$. Recall that $W_n$ denotes the nodes of $W$ that a node $n \in N$ covers. Let $I_{w, k-1}$ indicate the number of times node $w \in W$ is covered by the nodes $N_{k-1}$. Let $\delta_{n,k-1}$ be the marginal coverage of $W$ provided be node $n$ when $N_{k-1}$ nodes are included within the tour. That is:
% $$\delta_{n,k-1} := \{w \in W_n : I_{w, k-1} = 2\}$$

% Then the second (coverage) constraint in iteration becomes that we find a node $n^2$ such that $\delta_{n,k-1} \cap W_{n_2} =  \delta_{n,k-1}$. (We can also just compare cardinality).




% \textbf{Find the best swap!}
% After completing the above, check that no node can be removed while maintaining feasibility. It is possible that a swap we made allows for other nodes to be removed. Want to remove if removing will reduce the cost of the tour.


% We estimate the cost of each swap (maybe using Stringing/Unstringing method for TSP?). 
% We then can sort the potential swaps from least costly to most costly. We can identify the best swap by starting with the least costly swap and finding the first swap that is feasible. This first one is optimal to our optimization subproblem.

% \textbf{Updating after an iteration}
% Suppose we identify $n^2$ to add to the tour and $n^1$ to remove from the tour. Then, we must update all the sets and parameters used within the procedure.


% \begin{align}
%     p_{w, k} & = p_{w, k-1} + \Delta_{w n^1 n^2} \quad \forall \ w \in W \nonumber \\
%     r_k & = \max_{w \in W}{p_{w, k}} \nonumber \\
%     I_{w, k} & = \begin{cases}
%       I_{w, k-1} - 1  & w \in W_{n_1} \setminus W_{n_2} \\
%       I_{w, k-1} +1 & w \in W_{n_2} \setminus W_{n_1}\\
%       I_{w, k-1}  & \text{otherwise}
%     \end{cases} \quad \forall \ w \in W  \nonumber \\
% \end{align}


% Value is computed as the ratio between 
% the expected cost change, $\Delta z_1$, and the change in $z_2$ resulting from the swap. A swap with high value is indicative of a swap that can greatly improve $z_2$ with relatively little increase in cost $z_1$.
% % We have already computed the new value of \eqref{reformobj2} when checking feasibility of the swap.
% The change in $z_2$ can be computed from
% $$\max_{w \in W}{\ p_{w,k-1}+ v^0_{w}(v_{n_1w} - v_{n_2w}) / (\alpha_{w,k-1}*(\alpha_{w,k-1} - v_{w,n_1} + v_{n_2w}))} - \max_{w \in W} p_{k-1} $$
% We estimate the cost of the swap (change in $z_1$) as follows. Given a node $n \in N_{k-1}$, denote its predecessor in $C_{k-1}$ as $n-1$ and its successor $n+1$.
% Then the estimated cost change from swapping $n_1$ and $n_2$ is
% $$\hat{c}_{n_1-1,n_1+1}-(\hat{c}_{n_1-1,n_1}+\hat{c}_{n_1,n_1+1})+min_{m \in N_{k-1}} \{ \hat{c}_{m-1,n_2}+ \hat{c}_{n_2,m}- \hat{c}_{m-1,m}\}$$
% % $$c_{n_1-1,n_1+1}-(c_{n_1-1,n_1}+c_{n_1,n_1+1})-f_{n_1}+f_{n_2}+min_{m \in N_{k-1}} \{ c_{m-1,n_2}+ c_{n_2,m}- c_{m-1,m}\}$$
% If $n_1$ represents `no drop box' then the cost change estimate becomes:
% $$\min_{m \in N_{k-1}} \{ \hat{c}_{m-1,n_2}+ \hat{c}_{n_2,m}- \hat{c}_{m-1,m}\}$$
% If $n_2$ represents `no drop box' then the cost change estimate becomes:
% $$\hat{c}_{n_1-1,n_1+1}-(\hat{c}_{n_1-1,n_1}+\hat{c}_{n_1,n_1+1})$$





==> scrap.tex <==


\section{Coverage Model Formulation}
We introduce decision variables $x_{ij}$ that equal one if the collection route goes from $i \in N$ to $j \in N$, and zero otherwise. We introduce decision variables $y_i$ that equal one if location $i \in W$ is not covered by a drop box included in the tour.
%
Using these variables we define the objective functions. The first objective function $z_1 = \sum_{i \in N} \sum_{j \in N} c_{ij} x_{ij}$ captures the cost of the collection route. The second objective function $z_2 = \sum_{i \in W} w_i p_i y_i$ captures the weighted number of voters not covered by at least one ballot drop box.

The maximal covering tour formulation of the problem is then:
%
\begin{align}
    \underset{x,y}{\min} \ &   [ z_1 = \sum_{i \in N} \sum_{j \in N} c_{ij} x_{ij},\ z_2 = \sum_{i \in W} w_i  p_i y_i ]  \label{model:obj}\\
    \text{s.t.} \ 
    % & \sum_{j \in N} x_{ij} \leq 1 & \forall i \in N \\
    & \sum_{j \in N} x_{t j} = 1 & \forall \ t \in T \label{model:existing} \\
    & \sum_{i \in P} \sum_{j \in N} x_{ij} = n \label{model:number} \\
    & \sum_{i \in N} x_{ij} = \sum_{k \in N} x_{jk} & \forall \ j \in N \label{model:balance} \\
    & u_i - u_j +1 \leq (|T|+n - 1)( 1- x_{ij}) & \forall \ i \in N,\ j \in N,\ i,j \neq s \label{model:SEC} \\
    % \sum_{i \in S} \sum_{j \in S} x_{ij} \leq |S|-1 & \forall S \subset N : 2 \leq |S| < n+m+1 \\ % note this is p+1 as the hub 0 is considered as a stop so we locate and stop at p locations in this formulation
    & u_i \leq |T|+n - 2 & \forall \ i \in N \label{model:u_max}\\
    & 1-y_\ell \leq \sum_{i \in N_\ell} \sum_{j \in N} x_{ij} & \forall \ \ell \in W \label{model:coverage}\\
    & 2 \leq \sum_{i \in N^{'}_\ell} x_{ij} & \forall \ \ell \in W \label{model:basecoverage}\\
    & x_{ij} \in \{0,1\} & \forall \ i \in N, j \in N \label{model:xbin} \\
    & y_{i} \in \{0,1\} & \forall \ i \in W \label{model:ybin} \\
    & u_i \in \mathbb{Z}_{\geq 0} & \forall \ i \in N \label{model:uint}
\end{align}

% \textcolor{red}{We could change this to multiple coverage if so desired. }

The two objectives are introduced in \eqref{model:obj}.
The first objective $z_1$ is to minimize the cost of the collection route beginning and ending at $s$ and visiting each ballot box in the system.
For a given node $i \in N$, the value $\sum_{j \in N} x_{ij}$ can be 0 or 1. It is one if and only if $i$ is the city clerk office, an existing ballot box is at $i$, or a new ballot box is located at $i$.
The second objective is to minimize the number of potential voters that are not covered by a ballot box.
Constraint set \eqref{model:existing} ensures that the city clerk office and all exiting ballot boxes are included within optimal collection route.
Constraint \eqref{model:number} ensures that $n$ new ballot drop boxes are located.
Constraint set \eqref{model:balance} ensures that a collection route leaves a node if it enters the node. 
% node $j \in N$ is visited within the tour then the tour enters and leaves that node. \textcolor{red}{<- Explain better}.
Constraint set \eqref{model:SEC} are the subtour elimination constraints.
This requires an additional integer variable $u_i$ that captures the relative positions of the visited locations withing the collection route.
We choose this formulation over one with an exponential number of subtour elimination constraints (e.g., Dantzig-Fulkerson-Johnson formulation) as to make the implementation of such a model more straightforward for practitioners.
Constraint set \eqref{model:u_max} limits the number of potential solutions.
Constraint set \eqref{model:coverage} defines if a node in $W$ is not covered by a node included within the collection route.
Constraint set \eqref{model:basecoverage} ensures that each voter has minimal coverage provided by at least two drop boxes.
Constraint set \eqref{model:xbin} ensures an arc is traversed at most once in the collection route. 
Constraint set \eqref{model:ybin} ensures that a voter location is either covered or not.
Constraint set \eqref{model:uint} defines $u_i$ for all $i \in N$ as integer valued.

\section{Case Study 2 -  over worst case in each location}
%###########################
% These results come from ~\Box\Research\Elections\drop box\Milwaukee Case Study Raw Data\Results\20211210
%###########################


Milwaukee is the most populous municipality in the state of Wisconsin, and had approximately 315,483 registered voters prior to the general election held in November 2020 \cite{city_of_milwaukee_open_data_portal_2020_nodate}. We construct a case study of Milwaukee and investigate the location of ballot drop boxes using our proposed model.

We define the set of voter populations ($W$) to be the set of census block groups in Milwaukee \cite{milwaukee_county_census_2018}. 
Figure \ref{fig:estimatedpop} illustrates the different block group locations in Milwaukee as well as the estimated number of individuals over the age of 18 in each block group in Wisconsin. 
We let the set of potential drop box locations ($N$) be the locations of the following in Milwaukee: court houses, election administrative buildings, fire stations, libraries, police stations, CVS, and Walgreens. Figure \ref{fig:potential_locations} illustrates the locations of these 93 potential locations. We let an election administrative building to be the single required drop box location ($T$). 
We let the cost of locating a drop box at court houses, fire stations, or police stations to be \$6,000 to reflect the cost of a drop box without additional security measures. 
We let the cost of the single election administrative building in $T$ to be \$0 to model the case that a drop box already exists there.  
We let the cost of locating a drop box at all other locations to be \$10,000 to reflect the cost of both a drop box and a security camera with it.

\begin{figure}[hbt!]
    \centering
     \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.8\textwidth]{2020est18+population.png}
    \caption{Milwaukee block group locations. Color intensity reflects the estimated population of individuals 18 years of age or older.}
    \label{fig:estimatedpop}
    \end{subfigure}
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.8\textwidth]{potential_locations.png}
    \caption{Potential drop box locations within the City of Milwaukee. \\ }
    \label{fig:potential_locations}
    \end{subfigure}
\end{figure}

We estimate the variable cost of collecting ballots between two potential drop box locations as follows. 
We obtain estimates on the driving duration between each potential drop box location using Bing Maps.
We let the cost of each mile (calculated by assuming an average travel speed of 30 mph) to be fifty-six cents to reflect the current federal mileage reimbursement. 
We also let each hour spent collecting ballots have an opportunity cost of \$200 to reflect the potential benefit of completing other election tasks, such as security training, reviewing compliance of submitted ballots, or conducting marketing to increase voter turnout. 
We assume that a bipartisan team of two people will perform the collection route at a time.
Each year, we assume ballots are collected 10 times in total across all elections. 
We  
Lastly, we assume the cost of collecting ballots increases each year by two percent which is roughly the average historical inflation rate.
We then compute the net-present value over an assumed 15 year life of the ballot drop boxes to find the estimated cost of collecting ballots in today's dollars.

% We compute the cost per minute duration ($d$) of the collection route as follows:
% $$ d \times \frac{1 \text{ hour}}{\text{60 minutes}} \times\sum_{i=0}^{14} (1.02^i)\times 10\times [\frac{\$0.56}{\text{mile}}\times \frac{30  \text{ miles}}{\text{hour}} + 2 \text{ people}\times \frac{\$200}{\text{person hour}}] = 1201.316d$$
% \textcolor{red}{Change the 'opportunity cost' to 50?. Would result in more interesting results (336.65).}
% \textcolor{red}{Change the 'opportunity cost' to 200?. Would result in more interesting results (1201.316).}
% \textcolor{red}{Change the 'opportunity cost' to 100?. Would result in (600.658).}
% The first component readjusts the minute duration to hour duration.
% The second component calculates the net present value of the variable cost over 15 years (est. life of the drop boxes) assuming a 2\% inflation rate. The third component assumes that the ballots are collected 10 times per year from the drop boxes (for all elections). The next component is the cost. There is a cost per mile set by the federal government (56 cents) and we assume that the collection route is driven at a speed of 30mph on average. The second component of the cost is the opportunity cost of the election workers. This is set at $50$ per hour. This opportunity cost can represent the marginal cost to hire new workers and/or the added benefit of other potential tasks (e.g., security training).
% Cost per mile is equal to the true cost (mileage @0.56) and the opportunity cost of the time spent performing the collection route (idk like $200$).

We determine the set cover of each location ($N_w$) by identifying potential drop box locations that satisfy at least two of the following statements.
\begin{itemize}
    \item The time to walk from the location to the drop box is no more than 15 minutes.
    \item The time to drive from the location to the drop box is no more than 15 minutes.
    \item The time to use public transit (i.e., city bus) from the location to the drop box is no more than 30 minutes.
    \item The road distance between the location and the drop box is no more than 4 miles. This accounts for other modes of transit like biking or ride-sharing and accounts for data quality issues.
\end{itemize}
\vspace{-0.2cm}
The times and distances between each location in $W$ and the potential drop box locations is collected from Bing Maps. As a proxy, we use the center of each drop box location when calculating the set covers.

Lastly, we determine the parameters for the access function as follows. We divide each block group further into populations depending on if they have a vehicle available to them and the location of their work, if any. 
We collect estimates for vehicle availability \cite{united_states_census_bureau_means_2019} and work locations \cite{united_states_census_bureau_work_nodate} from the U.S. Census Bureau.
Figure \ref{fig:estimatedworklocations} illustrates the estimated number of individuals working in each census tract in Milwaukee County. The darker the color, the more individuals there. 
Figure \ref{fig:estimatedvehicleunavailablility} illustrates the intensity of vehicle availability within different block groups. Green indicates that a relatively high proportion of the population has access to a vehicle, while red indicates the opposite.

\begin{figure}[hbt!]
    \centering
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.8\textwidth]{work_locations.png}
    \caption{Estimated number of residents of the City of Milwaukee working in each census tract in Milwaukee County.\\ }
    \label{fig:estimatedworklocations}
    \end{subfigure}
    \hspace{0.05\textwidth}
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.8\textwidth]{no_vehicle_access.png}
    \caption{Proportion of residents in each census block group in the City of Milwaukee reporting they do not have a vehicle available to use.}
    \label{fig:estimatedvehicleunavailablility}
    \end{subfigure}
\end{figure}

We let $v^0_{w}$ and $v^1_{w}$ be determined by the estimated voter turnout among registered voters in each block group during the 2020 General election. Figure \ref{fig:estimatedvotingrate} illustrates the intensity of voting within the Milwaukee block groups. 
We let $v^1_{w}$ be equal to the voter turnout percentage and $v^0_{w}$ be equal to $100-v^1_{w}$.
We compute the parameter $v_{nw}$ for each potential drop box and for each voter subpopulation as follows to account for the benefit of drop boxes being near the location of the voters. 

$$ 5*\frac{100}{v^1_{w}}^2\sqrt[\leftroot{-2}\uproot{2}4]{\frac{1}{transit^4} + \frac{1}{walking^4} +\frac{1}{(4*roaddistance)^4}+\frac{\text{if car avail}}{drive^4} +\frac{\text{work != NA}}{work^4} }$$

\begin{figure}[hbt!]
    \centering
         \includegraphics[width = 0.24\textwidth]{2020estvotingrate.png}
    \caption{Estimated voting rate in the 2020 General election in each census block group within the City of Milwaukee.}
    \label{fig:estimatedvotingrate}
\end{figure}






% Manual changes - 
% \begin{enumerate}
%     \item Changed a negative 'None' value to 0.0001 (more people voted than there were registered voters) from -5.859375
% \end{enumerate}


% -------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------
% RESULTS
% -------------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------------------
\subsection{Results}

\newcommand\drawredsquare{%
\begin{tikzpicture}    
    \tikz\draw[red] (0,0) rectangle (1ex,1ex);  
  \end{tikzpicture}% 
}   

Selecting ballot drop boxes is non-trivial as demonstrated by our results. Figure \ref{fig:frontier} illustrates the approximate Pareto frontier (\ref{fig:frontier_cost}) obtained when solving the DBLP using the exact, epsilon constraint method.
Note this is not the complete frontier, but rather a subset of the points that lie on it.
Also plotted are the fixed cost (\ref{fig:frontier_fcost}) and variable cost (\ref{fig:frontier_vcost}) determined by the optimal solutions. In this figure, as the value on the horizontal axis increases, the minimal access function value increases. As the value on the vertical axis increases, the cost of managing the drop box system increases.
The solutions indicated by the red boxes (\protect\drawredsquare) are further explored in Figure \ref{fig:illustrate_tours}.
This figure illustrates the trade-off between increasing the coverage of populations within Milwaukee and the cost of the drop box system. However, the magnitude of the trade-off is not constant. When populations have relatively low access to the voting system, the marginal cost increase to improve the minimal access function value is small. When populations have relatively high coverage, the marginal cost of increasing the minimal access function value is high. The optimal solution defined by this frontier must be determined by the budget available to election administrators and equity/equality goals of an election jurisdiction.


\begin{figure}[!htb]
\centering
\captionsetup{width = 0.7\textwidth}
\begin{tikzpicture}
\begin{axis}[
	width=0.7\textwidth,
      height=0.4\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.5,-0.38)},anchor=south},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        % ylabel={\shortstack{Cost (\$) to locate \\and manage drop boxes}},
        ylabel={Cost},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={\shortstack{Minimum access function Value}},
        enlargelimits = true,
        legend columns = 3,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Total Cost ($z_1$)} \label{fig:frontier_cost}
      \addplot[const plot,mark=star,green] table [y=F,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Fixed Cost} \label{fig:frontier_fcost}
      \addplot[mark=*,blue] table [y=V,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Variable Cost} \label{fig:frontier_vcost}
      %
      \addplot[mark=square,mark size=4pt,mark options={color=red}] plot coordinates {(0.606524373626589,251109.957577)}; \label{fig:redbox}
      %
      \addplot[mark=square,mark size=4pt,mark options={color=red}] plot coordinates {(0.702291121854899,380408.7061342)};
      %
      \addplot[mark=square,mark size=4pt,mark options={color=red}] plot coordinates {(0.660748675432018,295886.024242999)};%
    %   \addplot[mark=star,red] table [y=P,x=F, col sep=comma]{frontier.dat};\addlegendentry{Fixed Cost} \label{fig:frontier_fcost}
      %
    %  \addplot[mark=square,blue-violet,blue] table [y=P,x=V, col sep=comma]{frontier.dat};\addlegendentry{Variable Cost}  \label{fig:frontier_vcost}
 \end{axis}
\end{tikzpicture}
\caption{\centering Approximate Pareto frontier of cost ($z_1^*$) versus minimum access function value. Also plotted are the fixed and variable costs making up the total cost. Solutions identified by (\protect\drawredsquare) indicate solutions explored in more detail in Figure \ref{fig:illustrate_tours}.} \label{fig:frontier}
\end{figure}

% \textcolor{red}{Compare to a solution that only considers fixed cost. What is the retrospective cost of each of these solutions (once we find TSP on them?)}


Table \ref{fig:frontier} presents the details of select optimal solutions on the approximate Pareto frontier, which correspond the the solutions on the frontier in Figure \ref{fig:frontier}.
Table \ref{fig:frontier} highlights the importance of considering both the fixed and variable cost of locating drop boxes, especially when the minimum access function value is low. 
For example, consider solutions 2, 3, and 4. Solution 4 provides the largest minimal access function value among the three solutions, but also the highest tour cost ($z_1$). However, solution 4 provides the lowest fixed cost among the three solutions. Thus, if the cost of collecting ballots was not determined when identifying solutions, solutions 2 and 3 would not be identified although they provide a lower total cost.


\begin{table}[!htb]
    \centering
    \caption{Select solutions. The solutions marked by (\protect\drawredsquare)  mark solutions identified on the Pareto frontier.}
    \label{T:dorian_value}
    \begin{tabular}{c c c c c c}
        % \ctoprule{3-7}
        \toprule
          \shortstack{Solution\\ID} & \shortstack{Minimum Access\\Function Value} & \shortstack{Tour\\Cost ($z_1$)} & \shortstack{Fixed\\Cost} & \shortstack{Variable\\Cost} & \shortstack{Num.\\ Drop Boxes} \\
         \midrule
0\lefteqn{\ (\protect\drawredsquare)}&0.607&251,109.96&96000&155,109.96&15\\
1&0.618&258,511.65&102000&156,511.65&16\\
2&0.628&269,092.25&112000&157,092.25&17\\
3&0.639&275,305.67&106000&169,305.67&16\\
4&0.650&283,912.79&108000&175,912.79&17\\
5\lefteqn{\ (\protect\drawredsquare)}&0.661&295,886.02&126000&169,886.02&18\\
6&0.671&311,817.27&150000&161,817.27&20\\
7&0.682&331,327.84&160000&171,327.84&23\\
8&0.692&354,251.01&180000&174,251.01&25\\
9\lefteqn{\ (\protect\drawredsquare)}&0.702&380,408.71&190000&190,408.71&28\\
10&0.712&406,646.62&218000&188,646.62&30\\
11&0.722&448,395.10&252000&196,395.10&35\\
12&0.733&499,380.60&280000&219,380.60&39\\
13&0.743&569,629.12&324000&245,629.12&45\\
14&0.753&674,747.99&412000&262,747.99&55\\
15&0.763&818,053.20&514000&304,053.20&66\\
16&0.773&1,107,310.78&696000&411,310.78&87\\
\bottomrule
    \end{tabular}
\end{table}

We explore three solutions in more detail. Figure \ref{fig:illustrate_tours} illustrates the selected drop box locations and the optimal tour visiting these drop boxes. Each black circle indicates a selected location for the drop box and the blue lines connecting each drop box describes the optimal collection route over these locations.
The color of each region indicates the access function values of each region (red means relatively poor coverage, green means relatively high coverage). 
We find that when cost is minimized (solution 0), drop boxes are generally well spaced in order to provide the double coverage to each location as is required by our formulation. In some instances, two drop boxes are located relatively close to each other. This occurs when both are required to ensure double coverage, but selecting locations near to each other leads to a low variable cost (tour length).
As the minimal value of the access function increases, we find that drop box locations are added to increase the coverage of populations that otherwise would be relatively uncovered. 
However, increasing the coverage of one location may cause another location to become the least covered location. 
We see this occur in solutions 5 and 9.
Thus, there is a non-trivial combinatorial trade-off to maximize coverage while meeting the constraints of the problem and minimizing the cost of the drop boxes. 



\begin{figure}[hbt!]
    \hspace{0.02\textwidth}
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.9\textwidth]{opt0.png}
    \caption{Solution 0}\label{fig:sol0}
    \end{subfigure}
    \hspace{0.02\textwidth}
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.9\textwidth]{opt5.png}
    \caption{Solution 5}
    \end{subfigure}
% \end{figure}
% \begin{figure}
    \centering
    \hspace{0.02\textwidth}
    \begin{subfigure}{0.3\textwidth}
     \includegraphics[width = 0.9\textwidth]{opt9.png}
    \caption{Solution 9}
    \end{subfigure}
\caption{Optimal drop box locations and tour visiting these locations. Color of regions reflect the access function value (red is low, green is high).}\label{fig:illustrate_tours}
\end{figure}

Despite these combinatorial challenges, we find that our proposed heuristic method approximates the Pareto frontier well and does so quickly.
Figure \ref{fig:frontier_compare} plots the approximate Pareto frontier found using the exact method (\ref{fig:frontier_exact}) against the approximate Pareto frontier found by our heuristic method (\ref{fig:frontier_heuristic}).
Computational studies were run on using 64 bit Python 3.7.7 on an Intel\textsuperscript{\textregistered} Core\textsuperscript{TM} i5-7500 CPU with 16 GB of RAM. The exact solution method was implemented using Gurobi 9.1.
We find that the exact method is able to generate 17 solutions on the Pareto frontier in 7 hours, while the heuristic method is able to generate 110 feasible (approximately Pareto) solutions in 90 seconds.
The main benefit of our proposed heuristic method is to highlight the trade-off between the minimum access function value and the cost of managing the drop box system ($z_1$) so that election officials can determine an appropriate location on the frontier to find an optimal solutions. Once an appropriate location on the Pareto frontier is selected, the optimal solution at that location can be solved relatively quickly. On average, the optimal solution can be found in approximately 30 minutes once the minimal allowable value for the access function is known.


\begin{figure}[H]%[!htb]
\centering
\captionsetup{width = 0.7\textwidth}
\begin{tikzpicture}
\begin{axis}[
	width=0.7\textwidth,
      height=0.4\textwidth,
      axis lines=middle,
      legend columns = 2,
      scaled y ticks=false,
        legend style={at={(0.5,-0.38)},anchor=south},
        legend cell align={left},
        x label style={at={(axis description cs:0.5,-0.12)},anchor=north},
        y label style={at={(axis description cs:-0.2,.5)},rotate=90,anchor=south},
        ylabel={Cost},
        yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
        },
        xlabel={\shortstack{Worst-case access function Value}},
        enlargelimits = true,
        legend columns = 3,
        % ymin = 150,
        % ymax= 500,
        % xmin = 0.4.
        % xmax = 0.7
          ] 
      \addplot[mark=triangle,black] table [y=C,x=P, col sep=comma]{frontier_mke.csv};\addlegendentry{Exact Method} \label{fig:frontier_exact}
      \addplot[const plot,red] table [y=C,x=P, col sep=comma]{frontier_heuristic_mke.csv};\addlegendentry{Heuristic Method} \label{fig:frontier_heuristic}
      %
 \end{axis}
\end{tikzpicture}
\caption{\centering Approximate Pareto frontier identified by the heuristic method compared to the exact solution method.} \label{fig:frontier_compare}
\end{figure}





\section{Extra intro}

\textcolor{red}{Deal with what is below}

There is often a trade-off between coverage drop boxes provide and the cost of the collection route. 
We highlight this trade-off using an example, depicted in Figure \ref{fig:example}.
% and Figure  \ref{fig:example_soln}.
% Figure \ref{fig:example_coverage} provides an example of the decision to be made. 
Suppose there are no drop boxes currently, there are five potential drop box locations, and the election administrator has sufficient funds to locate three new drop boxes. 
There are 12 voters that the election administrator aims to provide access to and the voters that each drop box covers is described using the gray ovals.
Figure \ref{fig:example_soln} provide two solutions to our problem and highlights the difference between the minimal length of the collection route and the maximal coverage of the drop boxes.
% have on the system. 
Figure \ref{fig:example_coverage} describes the optimal drop box locations when coverage of voters is maximized. 
The selected drop boxes are able to cover nine voters, but collection route has a length of 13 units.
Figure \ref{fig:example_cost} describes the optimal drop box locations when the collection route, or tour, is minimized.
The selected drop boxes are able to cover seven voters, but the collection route length is reduced to 6 units.
Existing guidelines only consider the access that the drop boxes provide to voting population. However, this may lead to a cost that may be infeasible in practice due to the time and resources it would require.
Moreover, in some cases, we may be able identify drop box locations that lead to a significantly shortened collection route while only slightly reducing the access provided to potential voters.
% ; our proposed optimization model can be used to find these solutions.
% Moreover, there may exist solutions that very slightly reduce the coverage of the voting-age population but significantly reduces the cost of managing the system. 
These solutions would enable election officials to spend additional time and resources providing other election services.
% Thus, the goal may not always be to increase access of ballot drop boxes to the voting aged individuals and cost must be taken into account.


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
     \includegraphics[width = \textwidth]{example_setup.png}
    \end{subfigure}
    \caption{Example problem with five potential drop box locations and 12 voter locations. The grey area surrounding each potential drop box indicates which voters the drop box covers. 
    The house is the start and end of the collection route.
    The goal is to select three drop boxes of the five that maximize the number of voters covered but also minimizes the tour length of collecting ballots at the drop boxes.
    }
    \label{fig:example}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.4 \linewidth}
     \includegraphics[width = \textwidth]{example_coverage.png}
     \caption{Maximize Coverage}\label{fig:example_coverage}
    \end{subfigure}
    \hspace{.1\linewidth}
    \begin{subfigure}[b]{0.4 \linewidth}
     \includegraphics[width = \textwidth]{example_cost.png}
     \caption{Minimize tour length} \label{fig:example_cost}
    \end{subfigure}
    \caption{The optimal drop box locations and the optimal tour visiting each selected drop box. When coverage is maximized (a), 9 voters are covered and the optimal tour length is 13. When tour length is minimized (b), coverage is 7 while tour length is 6.}
    \label{fig:example_soln}
\end{figure}


% \subsection{Project Significance}


This approach is similar to previously proposed facility location problems.
\citet{current_covering_1989} introduce the covering salesman problem, which aims to identify the least cost tour visiting $n$ cities from a larger number of possible cities such that
every city not included in the tour is within some predetermined distance from a city included in the tour.
\citet{gendreau_covering_1997} extend this problem to the covering tour problem such that the nodes that can be included in the tour and the nodes that must be covered are members of distinct sets.
\citet{current_median_1994} introduce the maximal covering tour problem as a bicriterion routing problem in which a tour visiting $p$ of $n$ potential nodes must be selected that minimizes the tour length and maximizes the coverage provided by the nodes selected to be within the tour to the nodes not within the tour. Applications identified by the authors include: mobile service delivery systems (e.g., rural health delivery), bi-modal transportation systems (e.g., overnight mail delivery), and distributed computer networks.
% They provide a heuristic method to produce solutions near the Pareto frontier.
% (this formulation isn't clear on how to deal with nodes that cannot be included in tour but must be 'covered' - although they do consider it in the case study...probably just fix certain variables to zero)

In our proposed research, we employ a maximal covering tour-based approach to maximize coverage of voters provided by drop boxes and minimize the length of the collection route to collect ballots from the drop boxes. Using this approach, we investigate the drop box system in a way that accounts for key aspects of the process that is often ignored by general guidelines. 
% \textcolor{red}{However, the problem formulation is founded on two NP-Hard problems (maximal coverage and traveling salesman problems). Significant effort is required to identify opportunities to reduce computational solution time.}

% Examples of this being used?

% Maybe talk about other election research?


% One of the most popular facility location approaches is to use ``coverage'' models, especially for service facilities \cite{farahani_covering_2012}.
% \citet{farahani_covering_2012} provide a literature review of covering problems in facility location problems from 1993 to 2011. 
% Set Covering Problem (SCP) vs Maximal Covering Location Problem (MCLP).
% SCP is to minimize location cost while ensuring a pre-specified level of service. Extensions include location set covering problen (LSCP), capacitated SCP, covering tour problem (CTP), path covering problems (might actually be interesting for this work, except reverse...being "covered" depends on typical travel pathways), probabilistic SCP, fizzy scp, multiple coverage scp, backup coverage scp (\url{https://scholar.google.com/scholar_lookup?title=Joint%20ground%20and%20air%20emergency%20medical%20services%20coverage%20models%3A%20A%20greedy%20heuristic%20solution%20approach&publication_year=2010&author=E.T.%20Erdemir&author=R.%20Batta&author=S.%20Spielman&author=P.A.%20Rogerson&author=A.%20Blatt&author=M.%20Flanigan}),
% non-cooperative covering games

% MCLP is to maximize coverage while locating a pre-specified number of facilities. planar maximal covering (locations are in 2D plane -- could be interesting), capacitated MCLP, MCLP with a criticality index analysis metric, MCLP with mandatory closeness constraints,Probabilistic MCLP, Maximum covering location-interdiction problem, Median Tour Problem (MTP) and Maximal Covering Tour Problem (MCTP) (this is related to the "cost" portion of the problem, actually might be the direct formulation we are interested, modified so county clerk office or where-ever is included in loop),Partial coverage problem, Generalized MCLP (GMCLP), Gradual coverage, Backup Coverage Location Problem (BCLP), p-Maximal cover problem, Quadratic MCLP, Complementary edge covering problem
% Public versus private sector applications

% Maximum Expected Coverage Location Problem (MEXCLP)  (where busy percent is probability that the drop-box is full)

% Bi-objective: primary and secondary coverage

% D.A. Schilling, vs. Jayaraman, R. Barkhi (1993)
% A review of covering problem in facility location




% Apply the covering tour problem to planning mobile healthcare facilities in Ghana
% https://onlinelibrary-wiley-com.ezproxy.library.wisc.edu/doi/abs/10.1111/0022-4146.00113


% Can't find version - application of the maximal covering tour problem
% https://www-tandfonline-com.ezproxy.library.wisc.edu/doi/abs/10.1080/01605682.2020.1746701

% They present a solution method for the bi-objective covering tour problem
% https://www-sciencedirect-com.ezproxy.library.wisc.edu/science/article/pii/S0305054805002480?via%3Dihub
% "Very few papers on the CTP have been published. Gendreau et al. [4] have proposed a model, a heuristic and a branch-and-cut algorithm for the CTP, and the latter has been applied successfully to the routing of a mobile medical facility in Ghana [6]. In addition, Maniezzo et al. [7] have presented a model and three scatter-search algorithms, and Motta et al. [8] have proposed a GRASP meta-heuristic for a generalized covering tour problem in which the nodes of W can also be visited."


% Papers to look at
% https://www-sciencedirect-com.ezproxy.library.wisc.edu/science/article/pii/S0968090X18307575

% \section{Lit Review?}
% Elections research?


\section{Extra lit review}


Locating polling locations:

\textcolor{red}{Deal with this stuff}
One of the most common approaches to facility location problems is to take a ``covering'' approach. With this approach, a location (e.g., voter) can be \textit{covered} by any one facility (e.g., drop box) within a predetermined subset of facilities. 
This is the approach we employ in our proposed research.
\citet{farahani_covering_2012} provide a literature review of covering problems in facility location problems from 1993 to 2011. They outline the main classes of problems: set covering problems and maximal covering location problem (MCLP).
With set covering problems, a minimum level of coverage must be met (e.g., 90\% of locations) and the goal is to minimize the number of needed facilities.
With maximal covering location problem, the number of facilities is fixed and the goal is to maximize coverage.
Numerous extensions have been proposed within the literature. 
%
In our proposed research, we employ a MCLP-based approach as an organization likely knows its budget and the number of drop boxes that they can afford before placing. Using this, we aim to best cover the voting-aged population.
However, in our approach we also consider the length, or \textit{cost}, of the collection route when deciding optimal drop box locations.
This collection route can alternatively be viewed as a \textit{tour} that begins, for example, at the city clerk's office, visits each drop box location, and returns to the city clerk's office.

\section{Extra heuristic}


We describe the process of identifying a new tour given a bound $r_k$ in the $k^\text{th}$ iteration.
\textcolor{red}{Instead of lowest cost, we take one with 'best value' (filtering out potential swaps that result in worse cost and participation.}

Before the initial iteration, we compute the following parameters:

$$\alpha_{w,0} := v^0_{w}+v^1_{w}+\sum_{j \in N_0} v_{nw} \quad \forall \ w \in W$$
$$p_{w,0} := v^0_{w} / \alpha_{w,0} \quad \forall \ w \in W$$
$$r_{0} :=  1 $$
$$r_{1} :=  \max_{w \in W} p_{w,0} $$
$$I_{w0} := |V_w \cap N_0 | \quad \forall \ w \in W$$

The $\alpha_{w,0}$ parameters represent the denominator of the access function given the inital tour nodes. 
The $p_{w,0}$ parameters represent the value of the access function for each $w\in W$ (Note that we consider 1-access function) for simplicity in calculations.
The $r_{0}$ parameter represents the value of the access function for the least covered population.
The $I_{w0}$ parameter represents the number of drop boxes that provide the base coverage (determined by the set covers) to location $w \in W$.
Given these initial parameters, the values of the access function can be incrementally updated throughout the procedure without needing to recompute the values in totality.

In the $k^\text{th}$ iteration, we take the following steps.
First, determine if a node in $N_{k-1}$ can be removed while maintaining (a) the double coverage of the each population and (b) drop box locations where the value of the access function for the least covered population is less than $r_k$. The feasibility of a node removal can be determined by checking the following statements:

$$ \max_{w \in W} p_{w,k-1}+ v^0_{w}v_{nw} / (\alpha_{w,k-1}*(\alpha_{w,k-1} - v_{w,n})) \leq r_{k} $$
$$\{w \in W_n : I_{w,k} = 2\} = \emptyset$$
\noindent These can be checked in $\mathcal{O}(|W|)$ time for each $n$.
%
% If there are multiple potential ``swaps'', determine which is estimated to reduce the cost of the tour the most.
If there are multiple potential node removals, determine which is estimated to reduce the cost of the tour the most.
Given a node $n \in N_{k-1}$, denote its predecessor as $n-1$ and its successor $n+1$. The most basic method to estimate this reduced cost is to compute the following $c_{n-1,n+1}-(c_{n-1,n}+c_{n,n+1})-f_n$ which estimates the cost increase of removing $n$ and adding an arc from its predecessor, $n-1$, to its successor, $n+1$.
% \textcolor{red}{What to do about the potential non-metric case?}
We then update the tour. This can be done using heuristics or exact methods. Since the number of drop boxes is relatives small, we compute an optimal tour over the selected drop box locations. Let $n$ be the node removed from the tour. We then update the parameters:

$$\alpha_{w,k} = \alpha_{w,k-1}- v_{nw} \quad \forall \ w \in W $$
$$p_{w,k} = p_{w,k-1}+ v^0_{w}v_{nw} / (\alpha_{w,k-1}*\alpha_{w,k}) \quad \forall \ w \in W$$
$$I_{w0} = \begin{cases}
      I_{w, k} - 1  & \text{if } w \in W_{n} \\
      I_{w, k}  & \text{otherwise}
    \end{cases} \quad \forall \ w \in W$$
$$N_{k} = N_{k} \setminus \{n_1\}$$
$$r_{k+1} =  \max_{w \in W} p_{w,k} $$
\noindent The parameters can be updated in $\mathcal{O}(|W|)$ time.

Let $c^*$ be the smallest change in cost after the previous steps ($c^* = \infty$ if no node can be removed). Next, we determine if a node currently visited by the tour can be removed and a node not currently visited by the tour can be added while increasing the cost of the tour by less than $c^*$.
The most basic method to estimate this reduced cost is to compute the following 
$$c_{n_1-1,n_1+1}-(c_{n_1-1,n_1}+c_{n_1,n_1+1})-f_{n_1}+f_{n_2}+min_{m \in N_{k-1}} \{ c_{m-1,n_2}+ c_{n_2,m}- c_{m-1,m}\}$$
If there are multiple potential ``swaps'', determine which is estimated to reduce the cost of the tour the most. We can check the feasibility of these swaps by checking if the following two statements are satisfied.
$$ \max_{w \in W} p_{w,k-1}+ v^0_{w}(v_{n_1w} - v_{n_2w}) / (\alpha_{w,k-1}*(\alpha_{w,k-1} - v_{w,n_1} + v_{n_2w})) \leq r_{k} $$
$$\{w \in W_{n_1} : I_{w,k} = 2\} \subseteq W_{n_2}$$
These conditions can be checked in $\mathcal{O}(|W|)$ time for each pairing $n_1$ and $n_2$. 
Let $n1$ denote the node that is removed from the tour and $n2$ denote the node added to the tour. Then we can update the parameters as follows:
$$\alpha_{w,k} = \alpha_{w,k-1}- v_{n_1w}+v_{n_2w} \quad \forall \ w \in W $$
$$p_{w,k} = p_{w,k-1}+v^0_{w}(v_{n_1w} -v_{n_2w}) / (\alpha_{w,k-1}*\alpha_{w,k}) \quad \forall \ w \in W$$
$$I_{wk} = \begin{cases}
      I_{w, k-1} - 1  &  \text{if }w \in W_{n_1} \setminus W_{n_2} \\
      I_{w, k-1} +1 &  \text{if } w \in W_{n_2} \setminus W_{n_1}\\
      I_{w, k-1}  & \text{otherwise}
    \end{cases} \quad \forall \ w \in W$$
$$N_{k} = N_{k} \cup \{n_2\} \setminus \{n_1\}$$
$$r_{k+1} =  \max_{w \in W} p_{w,k} $$
\noindent The parameters can be updated in $\mathcal{O}(|W|)$ time.

Let $c^*$ be the smallest change in cost after the previous steps ($c^* = \infty$ if no node can be removed).
Determine the drop box location not currently selected to add based on the estimated increase cost to the tour (both fixed and variable).
Assuming every $v_{wn} > 0$, it will be feasible to add any drop box location. If this is not true, we must simply verify that $v_{wn} > 0$ for the $w$ population with the worst access function value in the previous step. The cost can be estimated using the following calculation:
$$f_{n}+min_{m \in N_{k-1}} \{ c_{m-1,n}+ c_{n,m}- c_{m-1,m}\}$$
Let $n$ be the lowest cost node to add to the tour.
%
$$\alpha_{w,k} = \alpha_{w,k-1}+v_{n_2w} \quad \forall \ w \in W $$
$$p_{w,k} = p_{w,k-1}-v^0_{w}v_{n_2w} / (\alpha_{w,k-1}*\alpha_{w,k}) \quad \forall \ w \in W$$
$$I_{wk} = \begin{cases}
      I_{w, k-1} +1 &  \text{if } w \in W_{n_2}\\
      I_{w, k-1}  & \text{otherwise}
    \end{cases} \quad \forall \ w \in W$$
$$N_{k} = N_{k} \cup \{n_2\}$$
$$r_{k+1} =  \max_{w \in W} p_{w,k} $$


In each iteration, we may also want to allow a ``local search'' for an improve tour cost while potentially leading to a worst-case value for the access function. This can be done as follows. In each step outlined above, instead of setting $r_{k+1} =  \max_{w \in W} p_{w,k}$, we set:
$$r_{k+1} =  \max \{r_k - \varepsilon,\ \max_{w \in W} p_{w,k} \}$$
where $\varepsilon$ represents some minimal required change between iterations. In addition to this change, we add the following to allow for no nodes to be added, removed, or swapped from the tour.
If $r_{k-1} < r_{k}$ and lowest cost change identified in the previous steps are greater than zero, then we make no changes to the tour and make the upper bound tighter.

$$\alpha_{w,k} = \alpha_{w,k-1} \quad \forall \ w \in W $$
$$p_{w,k} = p_{w,k-1} \quad \forall \ w \in W$$
$$I_{w0} = I_{w, k} \quad \forall \ w \in W$$
$$N_{k} = N_{k}$$
$$r_{k+1} =  \max \{r_k - \varepsilon,\ \max_{w \in W} p_{w,k} \}$$


The steps above can complete in $\mathcal{O}(|W||N|^2)$ time. Once we have determined an actions to take from the above steps, we must update the tour based on the new nodes. 
In our implementation, we solve the TSP over $N_{k}$ to get the updated tour. This gives us the tour $\mathcal{C}_k$.
Generally, this solves quickly since the number of selected drop box  locations is small. If a polynomial time algorithm is desired, a heuristic or approximation algorithm for the TSP can be used instead of an exact method.

% \newcommand{\ubar}[1]{\text{\b{$#1$}}}
% \begin{algorithm}[H]
% \caption{Algorithm}\label{alg:cap}
% \textbf{Input}  An instance to DBLP
% \begin{algorithmic}[1]
% \State $N^0 \gets \text{Covering Tour Problem}(N,T,c,W,N_w)$ 
% \State $N^0 \gets \text{Covering Tour Problem}(N,T\cup N^0,c, W\setminus \{w \in W : N_w \cap N^0 \geq 2\},N_w \setminus N^0)$ 
% \State $\alpha_{w0} \gets v^0_{w}+v^1_{w}+\sum_{j \in N^0} v_{nw} \ \forall \ w \in W$
% \State $p_{w0} \gets v^0_{w} / \alpha_{w0}$
% % \frac{}{v^0_{w}+v^1_{w}+\sum_{j \in N^0} v_{nw}} \ \forall \ w \in W$
% \State $r_0 \gets \max_{w \in W} p_{w0} $
% \State $\text{Stop} \gets \max_{w \in W} \frac{v^0_{w}}{v^0_{w}+v^1_{w}+\sum_{j \in N} v_{nw}} $
% \State $k \gets 0$
% \State $I_{w,0} \gets |V_w \cap N_0| \ \forall \ w\in W$
% \While{$r_0 > \text{Stop}$} 
% \State $\beta \gets \infty$ \Comment{Best cost swap}
% \State $\beta_{\text{swap}} \gets \emptyset$\Comment{Best swap}
% \State $p_{w,k+1},\ I_{w,k+1},\ \alpha_{w,k+1},\ r_{k+1} \gets p_{w,k},\ I_{w,k},\ \alpha_{w,k},\ r_k$
% \For{$n_2 \in N\setminus N^{k}$} \Comment{Node to add}
%     \For{$n_1 \in N^{k}\setminus T$} \Comment{Node to remove}
%         \State $\hat{c}_{n_1,n_2} \gets \text{Estimate Cost Change} $ %c_{n_1 - 1, n_1+1} - c_{n_1 - 1, n_1} - c_{n_1, n_1+1} + \min_{n \in N^{k}\setminus}{c_{n,n2} + c_{n2,n+1}}$ \Comment{Need to fix}
%       \If{$\hat{c}_{n_1,n_2} <  \beta$} \Comment{We check feasibility}
%       \State $\delta \gets \{w \in W : I_{w,k} = 2\}$
%       \If{$\delta \cap W_{n_2} = \delta$} 
%       \State $\Delta_{w} \gets  v_{0,w}(v_{n_1,w}-v_{n_2,w})/(\alpha_{w,k}*(\alpha_{w,k}-v_{n_1,w}+v_{n_2,w})) \quad \forall \ w \in W$
%       \State $\hat{r} \gets \max{w \in W}  p_{w,k}+\Delta_w$
%       \If{ $\hat{r} < r_k $}
%       \State $r_{k+1} \gets \hat{r}$
%       \State $\beta \gets \hat{c}_{n_1,n_2}$
%       \State $\beta_{\text{swap}} \gets n_1,n_2$
%       \State $p_{w,k+1} \gets p_{w,k}+\Delta_w \ \forall \ w\in W $
%       \State $I_{w,k+1} \gets  \begin{cases}
%       I_{w, k} - 1  & w \in W_{n_1} \setminus W_{n_2} \\
%       I_{w, k} +1 & w \in W_{n_2} \setminus W_{n_1}\\
%       I_{w, k}  & \text{otherwise}
%     \end{cases} \quad \forall \ w \in W$
%         \EndIf
%         \EndIf
%         \EndIf
%     \EndFor
%     \State $\hat{c}_{n_2} \gets \text{Estimate Cost Addition}$ \Comment{Considering not removing any}
%     \If{$\hat{c}_{n_2} < \beta$}
%     \State $\Delta_{w} \gets  v_{0,w}(-v_{n_2,w})/(\alpha_{w,k}*(\alpha_{w,k}+v_{n_2,w})) \quad \forall \ w \in W$
%     %   \State $\hat{r} \gets \min_{w \in W}  p_{w,k}+\Delta_w$
%     %   \If{ $\hat{r} < r_k $}
%     %   \State $r_{k+1} \gets \hat{r}$
%       \State $r_{k+1} \gets \max{w \in W}  p_{w,k}+\Delta_w$
%       \State $\beta \gets \hat{c}_{n_2}$
%       \State $\beta_{\text{swap}} \gets n_1,n_2$
%       \State $p_{w,k+1} \gets p_{w,k}+\Delta_w \ \forall \ w\in W $
%       \State $I_{w,k+1} \gets  \begin{cases}
%       I_{w, k} +1 & w \in W_{n_2}\\
%       I_{w, k}  & \text{otherwise}
%     \end{cases} \quad \forall \ w \in W$
%         \EndIf
% \EndFor
% % \If{$\beta < 0$} \Comment{We have a swap to make.}
% % \EndIf
% \State $k \gets k + 1$
% % Updating the parameters
% \EndWhile
% \end{algorithmic}
% % \hspace*{\algorithmicindent} 
% \end{algorithm}


% Note that we only need only need to look at marginal coverage no longer provided by $n$ and the additional coverage offered by $n^*$. We Should be able to incremental coverage of $w$ and then see if what $n$ covers already has coverage greater than 2. If not, then $n^*$ must provide that incremental base coverage.

% This is a much smaller problem that we can solve by starting with the lowest cost swap and checking feasibility and progressing until we find a feasible solution.

% \textcolor{red}{Is there a way to update these without recomputing each iteration? Only base on some of the values. Yes there should be}

